Maintenance of Strongly Connected Component in Shared-memory Graph

In this paper, we present an on-line fully dynamic algorithm for maintaining strongly connected component of a directed graph in a shared memory architecture. The edges and vertices are added or deleted concurrently by fixed number of threads. To the best of our knowledge, this is the first work to propose using linearizable concurrent directed graph and is build using both ordered and unordered list-based set. We provide an empirical comparison against sequential and coarse-grained. The results show our algorithm's throughput is increased between 3 to 6x depending on different workload distributions and applications. We believe that there are huge applications in the on-line graph. Finally, we show how the algorithm can be extended to community detection in on-line graph.

==> conc-graph.tex <==

\section{Decremental Maintanance of SCC}
\label{sec:con-graph-ds}
\vspace{-1mm}
\subsection{Overview}
\label{sec:con-graph-ds:overview}
In this section we describe the graph data structure. It is based on the adjacency list representation. Hence, it is implemented as a collection (list) of vertices wherein each vertex in turn holds a list of vertices to which it has outgoing edges. The implementation is a linked list of \textit{\vnode} and \textit{\enode} as shown in the Table \ref{tab:struct:vertex-edge} (more details in \secref{app-con-graph-ds} of Appendix). The implementation of each of these lists are based on the lazy-list implementation of the a concurrent-set \cite{Heller-PPL2007}. 

\ignore{
The $\enode$ class has four fields. The $val$ field is the key value of the $edge(u,v)$ (edge from $u$ to $v$), stores the key value of $v$. The edge nodes are sorted in order of the $val$ field. This helps efficiently detect when a \textit{\enode} is absent in the edge list. The $marked$ field is of type boolean which indicates whether that \textit{\enode} is in the edge list or not. The $enext$ field is a reference to the next \textit{\enode} in the edge list. The $lock$ field is for ensuring access to a shared \textit{\enode} happens in a mutually exclusion manner. %We say a thread acquires a lock and releases the lock  when it executes a \textit{lock.acquire()} and \textit{lock.release()} method call respectively.

Similarly, the $\vnode$ class has six fields. The $val$ field is the key value of the vertex $u$. The vertex nodes are sorted in the order of the $val$ field which helps detect presence/absence of a \textit{\vnode} in the vertex list (like the the sorted \enode list). The $marked$ field is a boolean marked field indicating whether that \textit{\vnode} is in the vertex list or not. The $vnext$ field is a reference to the next \textit{\vnode} in the vertex list. The $\eh$ field is a sentinel \textit{\enode} at the start of the each edge list for each \textit{\vnode} has the smallest possible key value ($-\infty$). The $\et$ field is sentinel \textit{\enode} at the end of the each edge list has the largest possible key value ($+\infty$). The $lock$ field to add the mutual exclusion to a shared \textit{\vnode} implementation. We assume the $enext$ and $marked$ fields of the $\enode$ structure are atomic. Similarly, the $vnext$ and $marked$ fields of a $\vnode$ are atomic. %We say a thread  acquires a lock and releases the lock  when it executes a \textit{lock.acquire()} and \textit{lock.release()} method call respectively.    
}

%\ignore{
\begin{table*}[ht]
\centering
\scriptsize
\noindent\begin{tabular}{ m{4.5cm}| m{6cm} } 
%\label{struct:vertex-edge}
 \hline \\[-2ex]
  {Edge Node} &   {Vertex Node} \\ %[-2ex]   
   \hrule & \hrule\\[-2ex]
    \begin{verbatim}
class enode{
    /* unique value */
    int val; 
    /* pointer to the next enode */
    enode enext; 
    /* Marked indicates whether 
    this node is deleted or not. */
    boolean marked; 
    Lock lock; 
};
\end{verbatim}
    &
\begin{verbatim}
class vnode{
    /* a unique value */
    int val; 
    // pointer to the next vnode
    vnode vnext; 
    // Head & Tail values initialized to infinity
    enode EdgeHead, EdgeTail; 
    // Indicates whether this node is deleted or not
    boolean marked; 
    Lock lock;
};
\end{verbatim}
\hfill  \\[-2ex]
\hrule & \hrule\\[-2ex]
\end{tabular}
\captionsetup{font=scriptsize}
\caption{Structure of Vertex and Edge Node.}
\label{tab:struct:vertex-edge}
%}
\vspace{-7mm}
\end{table*}
%}
%\vspace{-5mm}
\ignore{
\noindent Given a global state $S$, we define a few structures and notations as follows: 
\begin{enumerate}
	\item We denote vertex node, say $v$, as a $\vnode$ class object. Similarly, we denote edge node, say $e$, as a $\enode$ class object.
    \item $\vnodes{S}$ as a set of $\vnode$ class objects that have been created so far in $S$. Its structure is defined in the Table \ref{tab:struct:vertex-edge}. Each $\vnode$ object $v$ in $\vnodes{S}$ is initialized with $key$, $vnext$ to $null$, $marked$ field initially set to $false$. Two sentinel edge nodes are created: $\eh$ and $\et$ assigned with val $-\infty$ and $+\infty$ respectively; $\et.enext$ to $null$ and $\eh.enext$ to $\et$.
    \item $\enodes{S}$ is a set of \enode class objects and its structure is defined in the Table \ref{tab:struct:vertex-edge}.  Each $\vnode$ object $v$ in $\enodes{S}$ is initialized with $key$, $enext$ to $null$, with $marked$ field initially set to $false$.
    \item $S.\vh$ is a $\vnode$ class object (called sentinel head vertex node), which is initialized with a val $-\infty$. This sentinel node is never removed from the vertex list. Similarly, $S.\vt$ is a $\vnode$ class object (called sentinel tail vertex node), which is initialized with a val $+\infty$. This sentinel node is never removed from the vertex list.
    %\item $S.\vt$ is a $\vnode$ class object (called sentinel tail vertex node), which is initialized with a val $+\infty$. This sentinel node is never removed from the vertex list.
    %\item For each $\vnode$ object $v$ in $\vnodes{S}$, two sentinel edge nodes are created: $\eh$ and $\et$ assigned with val $-\infty$ and $+\infty$ respectively. These structures can be seen in the Table \ref{tab:struct:vertex-edge}.
    \item The contents \& the status of a $\vnode$ $v$ keeps changing with different global states. For a global state $S$, we denote $S.v$ as its current state and the individual fields of $v$ in $S$ as $S.v.val, S.v.vnext, ...$ etc.  %$S.v$, $S.u$ are the S.\vnode of the graph $G$ for a global state $S$.
    \item Similar to the contents of a \vnode, it can be seen that the contents \& the status of a \enode $e$ keeps changing with different global states. Similarly, for a global state $S$, we denote $S.e$ as its current state and the individual fields of $e$ in $S$ as $S.e.val, S.e.vnext, ...$ etc.  %$S.v$, $S.u$ are the S.\vnode of the graph $G$ for a global state $S$.    
    %\item $S.e$ is the S.\enode of the graph $G$ for a global state $S$.
\end{enumerate}
 
 \noindent Having defined a few notions on $S$, we now define the notion of an abstract graph, $\abg$ for a global state $S$ which we will use for guiding us in correctness of our \mth{s}. $\abg$ for a global state $S$ is the collection of $S.\abgv$ and $S.\abge$ as defined below:
 
 \begin{definition}
\label{def:abgV}
	$S.\abgv \equiv \{v | (v \in \vnodes{S}) \land (S.\vh \rightarrow^* S.v) \land (\neg S.v.marked)\}$.
\end{definition}

\noindent This definition of \abgv captures the set of all vertices of $\abg$ for the global state $S$. It consists of all the \vnode{s} that are reachable from $S.\vh$ and are not marked for deletion. 

\begin{definition}
\label{def:abgE}
	$S.\abge \equiv \{e | (e \in S.enodes) \land ((u, v) \subseteq S.\abgv) \land (S.u.\eh \rightarrow^* S.e) \land (\neg S.e.marked) \land (S.e.val = S.v.val)\}$.
\end{definition}

\noindent This definition of $\abge$ captures the set of all edges of $\abg$ for the global state $S$. Informally it consists of all the $\enode$s that connects two $\vnode$s $u$, $v$ with the edge going form $u$ to $v$. 

}

The problems addressed in this paper are as follows: (1)  A concurrent directed graph $G = (V,E)$, which is dynamically being modified by a fixed set of concurrent threads. In this setting, threads may perform insertion / deletion of vertices or edges to the graph. We develop this data-structure in Section \ref{sec:working-con-graph-methods}. (2) We also maintain an invariant that the concurrent graph $G$ updated by concurrent threads should be acyclic. This means that the graph should preserve acyclicity at the end of every operation in the generated equivalent sequential history. We describe the modified data-structure in Section \ref{sec:Maintaining-Graph-Acyclicity}.  


\ignore{
\noindent The problems addressed in this paper are defined as here: 
\begin{enumerate}
\vspace{-1mm}
    \item A concurrent directed graph $G = (V,E)$, which is dynamically being modified by a fixed set of concurrent threads. In this setting, threads may perform insertion / deletion of vertices or edges to the graph. We develop this data-structure in Section \ref{sec:working-con-graph-methods}.
    \item We also maintain an invariant that the concurrent graph $G$ updated by concurrent threads should be acyclic. This means that the graph should preserve acyclicity at the end of every operation in the generated equivalent sequential history. We describe the modified data-structure in Section \ref{sec:Maintaining-Graph-Acyclicity}.  
\end{enumerate}
}
%\vspace{-5mm}
We assume that all the vertices have unique identification key (captured by $val$ field). Serialization Graph Testing Algorithm which is our motivating example, assumes that all the transactions have unique ids. Once a transaction is deleted it does not come back again into the system. As a result, we assume that all the vertices are assigned unique keys and duplicate vertices are not allowed. We assume that once a vertex id has been added, it will not be added again to the concurrent graph $G$. 
\vspace{-0.2cm}

\ignore{

\begin{table*}[th]
 \centering
  \captionof{table}{Sequential Specification of the Graph Data Structure } \label{tab:seq-spe} 
\begin{tabular}{ |m{3cm}|m{1cm}|m{5cm}|m{5cm}| } 

\hline
  \textbf{Method} & \textbf{Return Value} & \textbf{Pre-state}($S$: global state)  & \textbf{Post-state}( $S'$: future state of $S$ such that $S \sqsubset S'$)  \\ 
  
  \hline
	$\addv (u)$  & $true$ &$ S: \langle u \notin S.\abgv \rangle $ &$ S':\langle u \in S'.\abgv \rangle$	 \\
\hline 
	$\addv (u)$  & $false$ & Never the case	 &Never the case 	 \\
\hline 
	$\remv (u)$  & $true$ &$ S: \langle u \in S.\abgv \rangle$ &$ S':\langle u \notin S'.\abgv \rangle$	 \\
	\hline 
$\remv (u)$  & $false$ &$ S: \langle u \notin S.\abgv \rangle$ &Same as pre-state \\%$\forall S:(u \notin S.\abgv)$	 \\
	\hline 
	$\adde (u, v)$  & $true$ &$ S: \langle u,v \in S.\abgv \wedge  ((u,v) \in S.\abge \vee (u,v) \notin S.\abge ) \rangle$ & $ S':\langle (u,v \in S'.\abgv \wedge (u,v) \in S'.\abge \rangle$	 \\
	\hline 
	$\adde(u, v)$  & $false$ &$ S: \langle  u \notin S.\abgv \vee v \notin S.\abgv \rangle$ &Same as pre-state \\%$\forall S: ((u,v) \notin S.S(E).AbG)  \vee (u \notin S.\abgv) \vee (v \notin S.\abgv)$ 
	\hline 
	$\reme(u, v)$  & $true$ &$ S: \langle u,v \in S.\abgv \wedge  ((u,v) \in S.\abge) \vee (u,v) \notin S.\abge ) \rangle$ &$ S':\langle u,v \in S'.\abgv) \wedge (u,v) \notin S'.\abge \rangle$	 \\	
	\hline 
	$\reme(u, v)$  & $false$ &$ S: \langle u\notin S.\abgv \vee v\notin S.\abgv \rangle $ & Same as pre-state \\ %$\forall S:((u\notin S.\abgv) \vee (v\notin S.\abgv)) \vee ((u,v) \notin S.S(E).AbG)$	 \\	
	\hline 
	$\conv(u)$  & $true$ &$ S: \langle u \in S.\abgv \rangle$ &Same as pre-state \\%$\forall S:(u \in S.\abgv)$	 \\
	\hline 
	$\conv(u)$  & $false$ &$ S: \langle u \notin S.\abgv \rangle$ &Same as pre-state \\ %\forall S:(u \notin S.\abgv)$	 \\
	\hline 
	$\cone(u, v)$  & $true$ &$ S: \langle u,v \in S.\abgv \wedge  (u,v) \in S.\abge  \rangle$ & Same as pre-state \\%$\forall S:(u,v \in S.\abgv) \wedge (v \in S.S(E).AbG)$	 \\
	\hline 
	$\cone(u, v)$  & $false$ &$ S: \langle u\notin S.\abgv \vee v\notin S.\abgv \vee  (u,v) \notin S.\abge \rangle$ &same as pre-state	 \\
 
\hline

\end{tabular}
\end{table*}
}

\subsection{Methods Exported \& Sequential Specification}
\label{sec:con-graph-ds:methods}
\vspace{-1mm}
\noindent In this sub-section, we describe the \mth{s} exported by the concurrent directed graph data structure  along with their sequential specification. This specification as the name suggests shows the behavior of the graph when all the \mth{s} are invoked sequentially.
\noindent 
\begin{enumerate}
\item The $\addv(u)$ method adds a vertex $u$ to the graph, returning $true$. This follows directly from our assumption that all the vertices are assigned distinct keys. Once added, the method will never invoke addition on this key again.
\item The $\remv(u)$ method deletes vertex $u$ from the graph, if it is present in the graph and returns true. By deleting this vertex $u$, this method ensures that all the incoming and outgoing vertices of $u$ are deleted as well. If the vertex is not in the graph, it returns $false$. 
\item The $\adde(u, v)$ method adds a directed edge $(u, v)$ to the concurrent graph if the edge $(u, v)$ is not already present in the graph and returns $true$. If the edge is already in the graph it simply returns $true$. But if either the vertices $u$ or $v$ is not present, it returns $false$. Section \ref{sec:working-con-graph-methods} presents the construction of concurrent data structure based upon this specification.

%To maintain the graph acyclicity invariant which is described in section \ref{sec:Maintaining-Graph-Acyclicity}, we change the specification of the $\adde$ method as follows: if either the vertices $u$ or $v$ is not present, it returns $false$, like in the earlier case. Similarly, if the edge is already present in the graph, it returns $true$.
%If both the vertices $u$ \& $v$ are present and the edge is not in the graph already, this method tests to see if this edge $(u,v)$ will form a cycle in the graph by invoking $CycleDetect$ method. If it does not form a cycle, the edge is added and it returns $true$. Otherwise, it returns $false$. 

\item The $\reme(u,v)$ method deletes the directed edge $(u, v)$ from the graph structure if it is present and returns $true$. If the edge $(u, v)$ is not present in the graph but the vertices $u$ \& $v$ are in the graph it still returns $true$. But, if either of the vertices $u$ or $v$ is not present in the graph it returns $false$. 
\item The $\cone(u,v)$ returns $true$, if the graph contains the edge ($u,v$); otherwise returns $false$. 
\item The $\conv(u)$ returns $true$, if the graph contains the vertex $u$; otherwise returns $false$.
\end{enumerate}
%\vspace{-2mm}
% For the vnodes $u$ and $v$, we represent a particular $\enode$ $e$ as the edge $(u,v)$, from $u$ to $v$, such that $e.val$ = $v.val$. We assume that a typical application invokes significantly more contains \mth{s} (\textit{\cone} and \textit{\conv}) than the update \mth{s} (\textit{\addv, \remv, \adde, \reme}).
%\noindent Table \ref{tab:seq-spe} describes the sequential specification of each method formally in any given global state $S$ before the execution of the method and future state $S'$ after executing it sequentially. The \textit{Pre-state} is the shared state before $\inv$ event and the \textit{Post-state} is also the shared state just after the $\rsp$ event of a method, which is depicted in the Figure \ref{fig:exec/hist}.

==> correctness.tex <==
\ignore{
\section{Correctness of Concurrent Graph Object}
\label{sec:proof}

In this section, we try to formalise the proof of our concurrent graph data structure based on $\lp$ events of the methods. Most of the notations used here are derived from \cite{Vafeiadis-ppopp2006}.
%--------------------------------------------
\ignore{
\subsection{Specification}
\textbf{Edge Node Specification}
\paragraph{Edge Node:} We use the notion of \emph{ENode} which is same as \texttt{Entry} in \cite{Heller-PPL2007} and \texttt{ENode} in \cite{Vafeiadis-ppopp2006}. It is defined in the Table \ref{tab:struct:vertex-edge}

We use the notation that $e$ is a edge node or $ENode(e)$ denote that $e$ is an instance of the class $ENode$. For a global state $S$, we denote $S.enodes$ as the set of all edge nodes in $S$. If in state $S$, edge node $a$'s $enext$ is edge node $b$, then we say that $a$ points to $b$. In this case, we also denote $S.a\rightarrow S.b$. We say that a node $e$ is public in $S$ or $S.public(e)$ is true if some other node's $enext$ (say $a$) is $n$, i.e., $S.a \rightarrow S.n$. 

A edge node $e$ is initialized as follows: (1) $val$ is set $key$ passes through the constructor (2) $enext$ is set to $nil$ (3) $marked$ is set to $false$ (4) $lock$ is unlocked. 

Lazy-list based set implementation for edge list assumes that there is a edge $\eh$ and $\et$ nodes for each vertex once created and are never deleted. The value of key in $\eh$ is $-\infty$ and the value of key in $\et$ is $+\infty$. \\
%-----------------------------------------------------------------------------

\textbf{Vertex Node Specification}
\paragraph{Vertex Node:} We use the notion of \emph{VNode} which is same as \texttt{Entry} in \cite{Heller-PPL2007} and \texttt{VNode} in \cite{Vafeiadis-ppopp2006}. It is defined in the Table \ref{tab:struct:vertex-edge}

We use the notation that $v$ is a vertex node or $VNode(v)$ denote that $v$ is an instance of the class $VNode$. For a global state $S$, we denote $S.vnodes$ as the set of all vertex nodes in $S$. If in state $S$, vertex node $a$'s $vnext$ is vertex node $b$, then we say that $a$ points to $b$. In this case, we also denote $S.a\rightarrow S.b$. We say that a node $u$ is public in $S$ or $S.public(v)$ is true if some other node's $vnext$ (say $a$) is $n$, i.e., $S.a \rightarrow S.n$. 

A vertex node $v$ is initialized as follows: (1) $val$ is set $key$ passes through the constructor (2) $enext$ is set to $nil$ (3) $vnext$ is set to $nil$ (4) $marked$ is set to $false$ (5) $lock$ is unlocked. 

Lazy-list based set implementation for vertex list assumes that there is a vertex $\vh$ and $\vt$ nodes which are never deleted. The value of key in $\vh$ is $-\infty$ and the value of key in $\vt$ is $+\infty$. 
}

%\subsection{LP Notations}
%Consider an event $e$. Then we denote the global pre-state and post-state of this event as $PreE[e]$ \& $PostE[e]$ respectively. Similarly, for a method $m$, we denote the global pre-state (before its $\inv$ event) and post-state (after its \rsp event) as $PreM[m]$ \& $PostM[m]$ respectively.

\ignore{
\begin{enumerate}
\item $[\dots]$ $\rightarrow$ is the public state of $E$.

\item $\pree{i}$ $\rightarrow$ is the pre-state of the execution of the $\lp$ event of method $m_i$.
\item $\prem{i}$ $\rightarrow$ is the pre-state of the sequential history of method $m_i$.
\item $\poste{i}$ $\rightarrow$ is the post-state of the execution of the $\lp$ event of method $m_i$.
\item $\postm{i}$ $\rightarrow$ is the post-state of the sequential history of method $m_i$.
\item $\retm{i}$ $\rightarrow$ is the return value of the sequential history of method $m_i$.
\item $\rete{i}$ $\rightarrow$ is the return value of the $\lp$ event of the method $m_i$

\item $E^{S}$: is the sequential execution of methods. It is the partial order of all the methods such that $\forall m_i, m_j \in Method$ $\rsp_i$ $<$ $\inv_j$, where $m_i$ $<$ $m_j$.

\item $E^{H}$: is the concurrent execution of methods .It is the random execution of all the methods with interleaving of $\inv$ and $\rsp$, such that there exists a partial order among Linearizable Points. 

\end{enumerate}
}
%\item $r_1$, $r_2$ $\rightarrow$ are the reference node(\vnode/\enode).
%\item $S.v_1.val$, $S.v_2.val$ $\rightarrow$ through the reference \vnode ($v_1$,$v_2$) accessing the value of actual vertex node.
%\item $S.e_1.val$, $S.e_2.val$ $\rightarrow$ through the reference \enode ($e_1$,$e_2$) accessing the value of actual edge node. 

%\item Private Node. The newly created node(VNode/ENode) while adding a vertex by $\addv$ method or adding an edge by $\adde$ method for a given thread. This node is locally created.
%\item Public Node. The node(VNode/ENode) which is in the shared memory know as public node. For empty graph both Head and Tail node for vertex node. And $\eh$ and $\et$ for the edge list of each vertex.

 %\item $E^{S}$:Partial order of all the methods such that $\forall m_i, m_j \in Method$ $ret_i$ $<$ $inv_j$, where $m_i$ $<$ $m_j$.
 %\item For a history $H$, let the corresponding execution be denoted as \textit{E = H.Exec()}. Similarly for an execution $E$, let its history be denoted as \textit{H = E.Hist()};

  % \item $E^{H}$: It is the random execution of all the methods with interleaving of $invocations(inv)$ and $responds(resp)$, such that there exists a partial order among Linearizable Points(LPs). 
 %  \item $Complete(H)$: It is a $H$, where every method's $inv$ has a corresponding $resp$, except the last method, where for any method $m_i$ we add the $resp_{m_i}$ only if $LP_{m_i}$ has executed otherwise simple discard the method $m_i$.
%\item Concurrent Graph data structures, A concurrent graph data structure has a state, which is stored in the shared memory with \vnode{s} or \enode{s} objects. For each thread, it make available for use each methods the graph data structure supports. A thread executes a method by issuing an invocation event for it and a method terminates by executing a return response to the thread.



\ignore{
\begin{observation}
\label{lem:node-forever}
Consider a global state $S$ which has a node(ENode/VNode) $n$. Then in any future state $S'$ of $S$, $n$ is node($ENode/VNode$) in $S'$ as well. Formally, $\langle \forall S, S': (n \in S.nodes) \land (S \sqsubset S') \Rightarrow (n \in S'.nodes) \rangle$. \qed
\end{observation}

\noindent With this lemma, we assume that nodes once created do not get deleted (ignoring garbage collection for now). 

\begin{observation}
	\label{lem:node-val}
	Consider a global state $S$ which has a node($ENode/VNode$) $n$ which has been initialized with key $k$. Then in any future state $S'$ the value of $n$ does not change. Formally, $\langle \forall S, S': (n \in S.nodes) \land (S \sqsubset S') \Rightarrow (n \in S'.nodes) \land (S.n.val = S'.n.val) \rangle$. \qed
\end{observation}

\begin{observation}
	\label{lem:node-mark}
	Consider a global state $S$ which has a node($ENode/VNode$) $n$ which has marked. Then in any future state $S'$ the node $n$ stays marked. Formally, $\langle \forall S, S': (n \in S.nodes) \land (S.n.marked) \land (S \sqsubset S') \Rightarrow (S'.n.marked) \rangle$. \qed
\end{observation}

%----------------------------------------------------




%-----------------------------------------------------------------
\begin{corollary}
\label{cor:same-node:vertex}
There cannot exist two $VNode$s with the same key in the $S.\abgv$ of a particular global state $S$. \qed
\end{corollary}

\begin{corollary}
\label{cor:same-node:edge}
There cannot exist two $ENode$s with the same key in the $S.\abge$ of a vertex node $v$ of a particular global state $S$. \qed
\end{corollary}

%---------------------------------------------------------------
\begin{observation}
	\label{Obs:locate:vertex}
 Consider a global state $S$ which is the post-state of return event of the method $LocateVertex(key)$ invoked in the $\addv$ or $\remv$ methods. Suppose the $LocateVertex$ method returns $(v_1, v_2)$. Then in the state $S$, we have, 
	\begin{enumerate}
	\item $\langle (v_1, v_2) \subseteq S.\abgv \rangle$. %\in S.vnodes \rangle$ and  $(v_1, v_2)$ are the public vertex list nodes.
	\item ($S.v_1.locked$ = $true$) and ($S.v_2.locked$ = $true$) 
    \item $(S.v_1.vnext = S.v_2)$ %$(\neg S.v_1.marked$  $\land $  $\neg S.v_2.marked)$  and  \qed
\end{enumerate} 
\end{observation}
%---------------------------------------------------------
\begin{observation}
	\label{Obs:locate:edge}
 Consider a global state $S$ which is the post-state of return event of the method $LocateEdge(key_1, key_2)$ invoked in the $\adde$ or $\reme$ methods. Suppose the $LocateEdge$ method returns $(e_1, e_2)$. Then in the state $S$, we have, 
	\begin{enumerate}
	\item $\langle (e_1, e_2) \subseteq S.\abge \rangle$.% \rangle $ and  $(e_1, e_2)$ are the public edge list nodes of the vertex $node(key_1)$.
	\item ($S.e_1.locked$ = $true$) and ($S.e_2.locked$ = $true$) 
    \item $(S.e_1.enext = S.e_2)$.  %$(\neg (S.\abgv.node(key_1).marked) \land   \neg (S.\abgv.node(key_2).marked))$ and \\ $(\neg (S.\abge.e_1.marked) \land  \neg (S.\abge.e_2.marked))$  \qed
\end{enumerate} 
\end{observation}
%--------------------------------------------------------
\begin{lemma}
\label{lem:loc-ret:vertex}
Consider the global state $S$ which is the post-state of return event of the method $LocateVertex(key)$ invoked in the $\addv$ or $\remv$ methods. Suppose the $LocateVertex$ method returns references as $(r.v_1, r.v_2)$. Then in the state $S$, we have that $(S.r.v_1.val < key \leq S.r.v_2.val)$ for all nodes whose $vnext \neq null$.

\end{lemma}

\begin{proof}
Line \ref{lin:locv3} of $LocateVertex(key)$ method initialises $S.r.v_1$ to point to $\vh$. Also, $S.r.v_2$ $=$ $S.r.v_1.vnext$ by Line \ref{lin:locv4}. Now the last time Line \ref{lin:locv6} in the while loop is executed, we know that $S.r.v_1.val$ $<$ $S.r.v_2.val$. The node key does not change as known by Observation \ref{lem:node-val}. So, before execution of Line \ref{lin:locv9}, we know that $S.r.v_2.val$ $\geq$ $key$ and $S.r.v_1.val$ $<$ $S.r.v_2.val$. Since these references $VNode$s are belongs to $S.vnodes$, $S.v_1.val < key \leq S.v_2.val$. Also, be the Observation \ref{Obs:locate:vertex} vertex nodes $(v_1, v_2)$ are locked, do not change the key value and reachable from the $\vh$. Hence proved. \qed
\end{proof}
%--------------------------------------------------------

\begin{lemma}
\label{lem:loc-ret:edge}
Consider the global state $S$ which is the post-state of return event of the method $LocateEdge(key_1, key_2)$ invoked in the $\adde$ or $\reme$ methods. Suppose the $LocateEdge$ method returns references as $(r.e_1, r.e_2)$. Then in the state $S$, we have that \\ $(S.r.e_1.val < key_2 \leq S.r.e_2.val)$ for all nodes whose $enext \neq null$.

\end{lemma}


\begin{proof}
Similar argument like Lemma \ref{lem:loc-ret:vertex}.
%Line \ref{lin:loce3} of $LocateEdge(key)$ method initialises $S.\abge.r.e_1$ to point to $\vh$. Also, $S.r.v_2$ $=$ $S.r.v_1.vnext$ by Line \ref{lin:locv4}. Now the last time Line \ref{lin:locv6} in the while loop is executed, we know that $S.r.v_1.val$ $<$ $S.r.v_2.val$. The node key does not change as known by Observation \ref{lem:node-val}. So, before execution of Line \label{lin:locv9}, we know that $S.r.v_2.val$ $\geq$ $key$ and $S.r.v_1.val$ $<$ $S.r.v_2.val$. Since these references $VNode$s are belongs to $S.nodes$, $S.v_1.val < key \leq S.v_2.val$. Also, be the Observation \ref{Obs:locate:vertex} vertex nodes $(v_1, v_2)$ are locked, do not change the key value and reachable from the $\vh$. Hence proved. \qed

\end{proof}

%--------------------------------------------------------
\begin{lemma}
\label{lem:val-change:vertex}
For a $VNode$ $v$ in any global state $S$, we have that $\langle \forall v | (v \in S.vnodes) \land (v.vnext \neq null): (S.v.val < S.v.vnext.val) \rangle$. 
\end{lemma}

\begin{proof}
We prove by induction on all events in $E^H$ that change the $vnext$ field of the vertex node.\\[0.1cm]
\textbf{Base condition:} Initially, before the first event that changes the $vnext$ field, we know that ($\vh.key$ $<$ $\vt.key$) $\land$ $(\vh, \vt)$ $\in$ $S.vnodes$.\\[0.1cm] 
\textbf{Induction Hypothesis:} Say, upto $k$ events that change the $vnext$ field of any $VNode$, $(\forall n |( n \in S.vnodes)$ $\land$ ( $n.vnext \neq null$): ($S.n.val$ $<$ $S.n.vnext.val))$.\\[0.1cm]
\textbf{Induction Step:}
So, as seen from the code, the $(k+1)^{th}$ event which can change the $vnext$ field be only one of the following:
\begin{enumerate}
\item \textbf{Line \ref{lin:addv5}} of $\addv(key)$ method: by observing the code, we notice that the Line \ref{lin:addv5} can be executed only after the $LocateVertex$ method returns. Line \ref{lin:addv4} of the $\addv$ method creates a new node $v_3$ with value $key$. Line \ref{lin:addv5} then sets $v_{3}.vnext$ $=$ $v_2$. Since this event does not change the next field of any $VNode$ reachable from the $\vh$ of the vertex list, the lemma is not violated. 

\item \textbf{Line \ref{lin:addv6}} of $\addv(key)$ method: by observing the code, we notice that the Line \ref{lin:addv6} can be executed only after the $LocateVertex$ method returns. From Lemma \ref{lem:loc-ret:vertex}, we know that when locate returns then $v_1.val$ $<$ $key$ $\leq$ $v_2.val$. To reach Line \ref{lin:addv6} of $\addv$ method, Line \ref{lin:addv3} should ensure that $v_2.val$ $\neq$ $key$. This implies that $v_1.val$ $<$ $key$ $<$ $v_2.val$. From Observation~\ref{Obs:locate:vertex}, we know that $v_1.vnext$ = $v_2$. Also, the atomic event at Line \ref{lin:addv6} sets $v_1.vnext$ = $v_3$ where $v_3.val = key$. \\[0.1cm]
Thus from $v_1.val$ $<$ $v_3.val$ $<$ $v_2.val$ and $v_1.vnext$ = $v_3$, we get $v_1.val$ $<$ $v_1.vnext.val$. Since $(v_1, v_2)$ $\in$ $S.vnodes$ and hence, $S.v_1.val$ $<$ $S.v_1.vnext.val$.

\item \textbf{Line \ref{lin:remv5}} of $\remv(key)$ method: by observing the code, we notice that the Line \ref{lin:remv5} can be executed only after the $LocateVertex$ method returns. From Lemma \ref{lem:loc-ret:vertex}, we know that when $LocateVertex$ returns then $v_1.val$ $<$ $key$ $\leq$ $v_2.val$. To reach Line \ref{lin:remv5} of $\remv$ method, Line \ref{lin:reme3} should ensure that $v_2.val$ $=$ $key$. This implies that $v_1.val$ $<$ ($key$ $=$ $v_2.val$). From Observation~\ref{Obs:locate:vertex}, we know that $v_1.vnext$ = $v_2$. Also, the atomic event at Line \ref{lin:remv6} sets $v_1.vnext$ = $v_2.vnext$. \\[0.1cm]
We know from Induction hypothesis, $v_2.val < v_2.vnext.val$. Thus from $v_1.val$ $<$ $v_2.val$ and $v_1.vnext$ = $v_2.vnext$, we get $v_1.val$ $<$ $v_1.vnext.val$. Since $(v_1, v_2)$ $\in$ $S.vnodes$ and hence, $S.v_1.val$ $<$ $S.v_1.vnext.val$. \qed
\end{enumerate}
\end{proof}
%-----------------------------------------------------------------------------------
%--------------------------------------------------------
\begin{lemma}
\label{lem:val-change:edge}
For a edge node $e$ in any global state $S$, we have that $\langle \forall e \in S.enodes \land e.enext \neq null: S.e.val < S.e.enext.val \rangle$. 
\end{lemma}

\begin{proof}
Similar argument like Lemma \ref{lem:val-change:vertex}. \qed
\end{proof}
%-------------------------------------------------------------------------------------


\begin{lemma}
\label{lem:val-ret:vertex}
Consider the global state $S$ which is the post-state of return event of the method LocateVertex(key) invoked in the \addv or \remv methods. Suppose the LocateVertex method returns $(v_1, v_2)$. Then in the state $S$, there are no other vnodes, $v_p, v_q$ $\in$ S.vnodes such that $(S.v_1.val < S.v_p.val < key $ $\leq $ $ S.v_q.val < S.v_2.val)$. 
\end{lemma}

\begin{proof}
We already know from Observation \ref{Obs:locate:vertex} that when $LocateVertex(key)$ retuns, $S.v_1.val < key \leq S.v_2.val$. Suppose, ($\exists$ $v_p, v_q$ $\in$ $S.node$) such that $(S.v_1.val < S.v_p.val < key \leq S.v_q.val < S.v_2.val)$.
\begin{enumerate}
\item Assume there exists a $vnode$ $v_p$ is lying between $(v_1, v_2)$ $\in$ $S.vnode$. But as from Observation \ref{Obs:locate:vertex}, we know that when $LocateVertex$ returns then $S.v_1.vnext = S.v_2$. But this contradicts our initial assumption. So we know that $\nexists$ $v_p$ $\in$ $S.vnode$, between $(v_1, v_2)$ such that ($S.v_1.val < S.v_p.val < key \leq S.v_2.val$).
\item Assume $\exists$ $v_p, v_q$ $\in$ $S.vnode$ such that $\vh$ $\rightarrow^*$ $v_p$ $\rightarrow$ $v_1$ $\rightarrow$ $key$ $\rightarrow$ $v_2$ $\rightarrow$ $v_q$ $\rightarrow^*$ $\vt$ such that $S.v_1.val < S.v_p.val < key \leq  S.v_q.val < S.v_2.val$. This means that, $(v_p.val > v_1.val) \land (v_p.vnext = v_1)$. But from Lemma \ref{lem:val-change:vertex}, we know that $\forall n \in S.vnodes: S.vnext$ $<$ $S.vnext.val$. This contradicts $(S.v_p.vnext = S.v_1) \land (S.v_p.val < S.v_1.val)$.
\end{enumerate}
Hence $\nexists$ $v_p, v_q$ $\in$ $S.vnodes$ such that $(S.v_1.val < S.v_p.val < key \leq S.v_q.val < S.v_2.val)$.
\qed
\end{proof}

\begin{lemma}
\label{lem:val-ret:edge}
Consider the global state $S$ which is the post-state of return event of the method $LocateEdge(key_1, key_2)$ invoked in the \adde or \reme methods. Suppose the $LocateEdge$ method returns $(e_1, e_2)$. Then in the state $S$, there are no other enodes, $e_p, e_q$ in $S.enodes$ of the vertex $vnode(key_1)$ such that $(S.e_1.val < S.e_p.val < key \leq S.e_q.val < S.e_2.val)$. 
\end{lemma}
\begin{proof}
Similar argument like Lemma \ref{lem:val-ret:vertex}. \qed
\end{proof}

\begin{lemma}
\label{lem:nonmark-reach:vertex}
	In a global state $S$, any non-marked public vnode $v$ is reachable from $\vh$. Formally, $\langle \forall v |
 (v \in S.vnodes) \land (\neg S.v.marked) \implies (\vh \rightarrow^* S.v) \rangle$. 
\end{lemma}

\begin{lemma}
\label{lem:nonmark-reach:edge}
	In a global state $S$, any non-marked public enode $e$ is reachable from $\vh$. Formally, $\langle \forall e |
 (e \in S.enodes) \land (\neg S.e.marked) \implies (\vh \rightarrow^* S.e) \rangle$. 
\end{lemma}


\begin{lemma}
\label{lem:change-abg}
	Only the events $write(v_1.vnext, v_3)$ in Line \ref{lin:addv6} of $\addv$,  $write(v_2.marked, true)$ in Line \ref{lin:remv4} of $\remv$, $write(e_1.enext, e_3)$ in Line \ref{lin:adde6} of $\adde$ and $write(e_2.marked, true)$ \ref{lin:reme4} of $\reme$ method can change the $\abg$.
\end{lemma}
\begin{proof}
It is to be noted that the $LocateVertex$, $LocateEdge$, $\conv$ and $\cone$ methods do not have any update events. By observing the code, it appears that the following events of the $\addv$, $\remv$, $\adde$ and $\reme$ methods can change the $\abg$:

\begin{enumerate}

\item \textbf{Line \ref{lin:addv4} \& \ref{lin:addv5} of $\addv(key)$} method:  In Algorithm~\ref{alg:add:Vertex}, let $S_1.\abgv$ be the initial state of the $\abgv$, such that we know from Line \ref{lin:addv3} that $key$ $\notin$ $S_1.\abgv$. Line \ref{lin:addv4} of the $\addv$ method creates a $vnode$ $v_3$ with value $key$, i.e. $v_3.val = key$. Now, Line \ref{lin:addv5} sets $v_3.vnext$ $=$ $v_2$. Since this event does not change the $vnext$ field of any  $vnode$ reachable from the $\vh$ of the vertex list ($v_3 \notin$ $S.Public(v)$), hence from Definition \ref{def:abgV}, $S_1.\abgv$ remains unchanged after these events.

\item \textbf{Line \ref{lin:addv6} of $\addv(key)$} method: At Line \ref{lin:addv3}, $true$ evaluation of the condition leads to the execution of $v_1.vnext = v_3$ at Line \ref{lin:addv6}. Also, $v_1$ and $v_2$ are locked, therefore from Observation \ref{Obs:locate:vertex}, $\vh$ $\rightarrow^*$ $v_1$. From Line \ref{lin:addv5} \& \ref{lin:addv6} we get: $v_1$ $\rightarrow$ $v_3$ $\rightarrow$ $v_2$. Hence, $\vh$ $\rightarrow^*$ $v_1$ $\rightarrow$ $v_3$ $\rightarrow$ $v_2$ follows. We have $\neg$ $(v_3.marked)$ $\land$ $(\vh$ $\rightarrow^*$ $v_3)$ $\land$ ($v_3$ $\in$ $S.Public(v)$). Thus from Definition \ref{def:abgV}, $S_1.\abgv$ changes to $S_2.\abgv$ $=$ $S_1.\abgv$ $\cup$ $v_3$.

\item \textbf{Line \ref{lin:remv4} of $\remv(key)$} method: By observing the code, we notice that the state before execution of Line \ref{lin:remv4} satisfies that $key$ $\in$ $S.\abgv$. After execution of Line \ref{lin:remv4}, $\abgv$ changes such that $key$ $\notin$ $S.\abgv$. Note that this follows from Definition \ref{def:abgV}.

\item \textbf{Line \ref{lin:remv5} of $\remv(key)$} method: Till Line \ref{lin:remv4} of the $\remv$ method, $S.\abgv$ has changed such that $v_2.val$ $\notin$ $S.\abgv$. So even after the execution of Line \ref{lin:remv5} when $v_1.vnext$ is set to $v_2.vnext$, $S.\abgv$ remains unchanged (from Definition \ref{def:abgV}).

\item \textbf{Line \ref{lin:adde4} \& \ref{lin:adde5} of $\adde(key_1, key_2)$} method:  In Algorithm~\ref{alg:add:Edge}, let $S_1.\abge$ be the initial state of the $\abge$, such that we know from Line \ref{lin:adde3} that $key_2$ $\notin$ $S_1.\abge$ of the vertex $vnode(key_1)$. Line \ref{lin:adde4} of the $\adde$ method creates a $enode$ $e_3$ with value $key_2$, i.e. $e_3.val = key_2$. Now, Line \ref{lin:adde5} sets $e_3.enext$ $=$ $e_2$. Since this event does not change the $enext$ field of any  $enode$ of the $vnode(key_1)$ reachable from the $\vh$ of the edge list ($v_3 \notin$ $S.Public(v)$), hence from Definition \ref{def:abgE}, $S_1.\abge$ remains unchanged after these events.

\item \textbf{Line \ref{lin:adde6} of $\adde(key_1, key_2)$} method: At Line \ref{lin:adde3}, $true$ evaluation of the condition leads to the execution of $e_1.enext = e_3$ at Line \ref{lin:adde6}. Also, $e_1$ and $e_2$ are locked, therefore from Observation \ref{Obs:locate:edge}, $\vh$ $\rightarrow^*$ $e_1$. From Line \ref{lin:adde5} \& \ref{lin:adde6} we get: $e_1$ $\rightarrow$ $e_3$ $\rightarrow$ $e_2$. Hence, $\vh$ $\rightarrow^*$ $e_1$ $\rightarrow$ $e_3$ $\rightarrow$ $e_2$ follows. We have $\neg$ $(e_3.marked)$ $\land$ $(\vh$ $\rightarrow^*$ $e_3)$ $\land$ ($e_3$ $\in$ $S.Public(e)$). Thus from Definition \ref{def:abgE}, $S_1.\abge$ changes to $S_2.\abge$ $=$ $S_1.\abge$ $\cup$ $e_3$.

\item \textbf{Line \ref{lin:reme4} of $\reme(key_1, key_2)$} method: By observing the code, we notice that the state before execution of Line \ref{lin:reme4} satisfies that $key_2$ $\in$ $S.\abge$ of the vertex $vnode(key_1)$. After execution of Line \ref{lin:reme4}, $\abge$ changes such that $key_2$ $\notin$ $S.\abge$ of the vertex $vnode(key_1)$. Note that this follows from Definition \ref{def:abgE}.

\item \textbf{Line \ref{lin:reme5} of $\reme(key_1, key_2)$} method: Till Line \ref{lin:reme4} of the $\reme$ method, $S.\abge$ has changed such that $e_2.val$ $\notin$ $S.\abge$ of the vertex $vnode(key_1)$. So even after the execution of Line \ref{lin:reme5} when $e_1.vnext$ is set to $e_2.enext$, $S.\abge$ remains unchanged (from Definition \ref{def:abgE}).


\end{enumerate}


Hence, only the events in Line \ref{lin:addv6} of $\addv$ method, in Line \ref{lin:remv4} of $\remv$ method, in Line \ref{lin:adde6} of $\adde$ and \ref{lin:reme4} of $\reme$ method can change the $\abg$. \qed

\end{proof}

\begin{corollary}
\label{cor:change-abg}
The events $write(v_1.vnext, v_3)$ of $\addv$, $write(v_2.marked, true)$ of $\remv$, $write(e_1.enext, e_3)$ of $\adde$ and $write(e_2.marked, true)$ of $\reme$ method  which change the $\abg$ are the Linearization Points(LPs) of the respective methods. \qed
\end{corollary}
}

\begin{figure}[H]
\centerline{\scalebox{0.7}{\input{figs/ConExe.pdf_t}}}
\caption{Figure (a) illustrates an example of a concurrent execution $E^H$. Then, $m_i.LP$ is the LP event of the method $m_i$. The global state immediately after this event is represented as Post-state of ($E^H.m_i.LP$). Figure (b) represents sequential execution $E^S$ corresponding to (a) with post-state of method $m_i$ as the state after its $\rsp$ event.}
\label{fig:conc:seq}
\end{figure}


\subsection{Safety: Proof Skeleton}
\noindent In this subsection, we describe the lemmas to prove the correctness of our concurrent graph data structure. 

\begin{observation}
\label{obs:change-abs}
	Only the \lp events in the execution can change the \abg. \qed
\end{observation}

\begin{lemma}
\label{lem:seqe-pre}
The global state of the graph after the \rsp event of a method is the same as the state before the \inv event of the consecutive method in the sequential execution. Formally, $\langle \postm{i}= \prem{i+1}\rangle$
\end{lemma}

\begin{proofsketch}
From the definition of Sequential Execution as depicted in Figure \ref{fig:conc:seq}(b).
\end{proofsketch}

\begin{lemma}
\label{lem:conce-pre}
In every concurrent execution ordered by its events, the global state of the graph immediately after a \lp event is the same as the state before the next \lp event. Formally, $ \langle \poste{i} = \pree{i+1} \rangle$
\end{lemma}

\begin{proofsketch}
\ignore{Let us prove by contradiction. Assume that there exists a method $m_k$ which modifies the $\abg$ between method $m_i$ and $m_{i+1}$.
As we know from the code that the events $write(v_1.vnext, v_3)$ in Line \ref{lin:addv6} of $\addv$,  $write(v_2.marked, true)$ in Line \ref{lin:remv4} of $\remv$, $write(e_1.enext, e_3)$ in Line \ref{lin:adde6} of $\adde$ and $write(e_2.marked, true)$ \ref{lin:reme4} of $\reme$ method can change the $\abg$ only. Any other events between the post-state of $E.m_i.\lp$ and the pre-state of $E.m_{i+1}.\lp$ will not change the $\abg$. Hence Proved.} From Observation \ref{obs:change-abs} as illustrated by Figure \ref{fig:conc:seq}(a).
\end{proofsketch}

%\ignore{
\begin{lemma}
\label{lem:conce-seqe-mi}
If the pre-state of a \lp event in the concurrent execution is the same as the pre-state of a method in sequential execution, then the post-state of the \lp event in concurrent execution must be same as the post-state of the method in sequential execution. Formally,
$ \langle(\pree{i} = \prem{i})\Longrightarrow (\poste{i} = \postm{i}) \rangle$.
\end{lemma}

\begin{proofsketch}
From Observation \ref{obs:change-abs}, we know that there is only one event which can change $AbG$ i.e. $\lp$. Given that the pre-states are same, only $\lp$ event gets executed in the execution (which is an atomic event), then on execution in sequential and concurrent execution, post-state remains same.
\end{proofsketch}

\begin{lemma}
\label{lem:conce-seqe-pre}
In every execution, we know that pre-state of \lp event must be same as the pre-state of the method in the sequential execution. Formally,
$\langle \pree{i} = \prem{i} \rangle$.
\end{lemma}

%\ignore{
\begin{proofsketch}
We prove by Induction on events which are the linearization points of the methods,\\[0.1cm]
\textbf{Base Step:} Before the $1^{st}$ $\lp$ event, the initial $\abg$ remains same because all the events in the concurrent execution before the $1^{st}$ $\lp$ do not change $\abg$.\\[0.3cm]
\textbf{Induction Hypothesis}: Let us assume that for $k$ $\lp$ events, we know that,\\[0.2cm]  
$\pree{k} = \prem{k}$ \\[0.3cm]
\textbf{Induction Step:} We have to prove that: $\pree{k+1} = \prem{k+1}$ holds true.\\[0.3cm]
We know from Induction Hypothesis that for $k^{th}$ method,\\[0.3cm]
$\pree{k} = \prem{k}$\\[0.3cm]
Now we know $\lp$ is an atomic event that is same in $E^H$ and $E^S$. From the Lemma \ref{lem:conce-seqe-mi} we have,
\begin{equation} 
\begin{split}
\label{lab:eq:conce-seqe-mi}
 (\pree{k} = \prem{k}) \xRightarrow[]{\text{From Lemma \ref{lem:conce-seqe-mi}}}\\ (\poste{k} = \postm{k})
 \end{split}
\end{equation} 

From the Lemma \ref{lem:seqe-pre}, we have,

\begin{equation} 
\label{lab:eq:seqe-pre}
 \postm{k} \xRightarrow[]{\text{From Lemma \ref{lem:seqe-pre}}}  \prem{k+1} 
\end{equation} 

From the equation \ref{lab:eq:conce-seqe-mi}
we have,
\begin{equation} 
\label{lab:eq:seqe-mi-post}
 \poste{k} =  \postm{k}
\end{equation} 

By combining the equation \ref{lab:eq:seqe-mi-post} and \ref{lab:eq:seqe-pre} we have,

\begin{equation} 
\label{lab:eq:seqe-mi-pre}
 \poste{k} =  \prem{k+1}
\end{equation} 

And from the Lemma \ref{lem:conce-pre} we have, \begin{equation} 
\label{lab:eq:conce-pre}
 \poste{k} =  \pree{k+1}
\end{equation}

So, by combining equations \ref{lab:eq:conce-pre} and \ref{lab:eq:seqe-mi-pre} we get,

\begin{equation} 
\label{lab:eq:conce-seuq-pre}
 \pree{k+1} =  \prem{k+1}
\end{equation}

Finally, $\pree{k+1} = \prem{k+1}$.\\[0.3cm]
Hence this holds for all $m_i$ in $E^H$. Hence Proved.

\end{proofsketch}
%}

\begin{lemma}
\label{lem:addVT-conc}
If some $\addv(key)$ method returns true in $E^H$, then the vertex node corresponding to that key will not be present in the pre-state of the \lp event of the method. Formally, \\ $\langle \addv(key, true) \Longrightarrow (\vnode(key) \notin \pree{i} \rangle$.
%\textit{ OR } \\ (vnode(key) \in ([E^{H}.Pre(\lin{m_{i}})].\abg)) \rangle$. 
\end{lemma}

\begin{proofsketch}
%\begin{enumerate}
%    \item $(vnode(key) \notin ([E^{H}.Pre(\lin{m_{i}})].\abg))$ :\\
By observing the code, we know from Line \ref{lin:addv2}, that when $LocateVertex(key)$ returns, vertex nodes $v_1$ and $v_2$ are locked, ($v_1, v_2$) $\in$ $\vnodes{S}$ and $v_1.val$ $<$ $key$ $\leq$ $v_2.val$. We know that $\lp$ of this method is Line \ref{lin:addv6}, which is reachable only by evaluating condition on Line \ref{lin:addv3} as $true$. This means $v_2.val$ $\neq$ $key$ and $v_2$ $\in$ $\vnodes{S}$, we know  $\vnode(key)$ belongs to $S.\abgv$, where $S.\abgv$ is the pre-state of the $LP$ event of the method and the key value of the $\vnode(key)$ doest not change after initialization. Hence, $\vnode(key)$ $\notin$ $\pree{i}$.
% \item $(vnode(key) \in ([E^{H}.Pre(\lin{m_{i}})].\abg))$:\\
% From Line \ref{lin:addv2}, when $LocateVertex$ returns we know that from Observation \ref{Obs:locate:vertex} \& Lemma \ref{lem:nonmark-reach:vertex}), $vnode$s $v_1$ and $v_2$ are locked and ($v_1, v_2$) $\in$ $S.vnodes$ and $v_1.val$ $<$ $key$ $\leq$ $v_2.val$. Now in Line \ref{lin:addv3}, $v_2.val$ $=$ $key$ is evaluated to $true$ such that $v_1.vnext = v_2$ and $v_2$ $\in$ $S.vnodes$, we know  $vnode(key)$ is belong to $S.\abgv$, where $S.\abgv$ is the pre-state of the $LP$ event of the method. Hence $vnode(key)$ $\in$ $([E^{H}.Pre(\lin{m_{i}})].\abg)$.
%\end{enumerate}
\end{proofsketch}

\begin{lemma}
\label{lem:removeVT-conc}
If some $\remv(key)$ method returns true in $E^H$, then the vertex node corresponding to that key must be present in the pre-state of \lp event of the method. Formally, \\ $\langle \remv(key, true) \Longrightarrow (\vnode(key) \in \pree{i} \rangle$
\end{lemma}

\begin{proofsketch}
By observing the code, we know from Line \ref{lin:remv2}, that when $LocateVertex(key)$ returns, vertex nodes $v_1$ and $v_2$ are locked, ($v_1, v_2$) $\in$ $\vnodes{S}$ and $v_1.val$ $<$ $key$ $\leq$ $v_2.val$. We know that the $\lp$ of this method is Line \ref{lin:remv4}, which is reachable only by evaluating the condition in Line \ref{lin:remv3} to $true$. This means that $v_2.val$ $=$ $key$ is evaluated to $true$ such that $v_1.vnext = v_2$ and $v_2$ $\in$ $\vnodes{S}$. Thus we know $\vnode(key)$ belongs to $S.\abgv$, where $S$ is the pre-state of the $\lp$ event of the method. Hence $\vnode(key)$ $\in$ $\pree{i}$.
\end{proofsketch}


\begin{lemma}
\label{lem:removeVF-conc}
If some $\remv(key)$ method returns false in $E^H$, then the vertex node corresponding to that key will not present in the pre-state of the LP event of the method. Formally, \\ $\langle \remv(key, false) \Longrightarrow (\vnode(key) \notin \pree{i} \rangle$.
 
\end{lemma}

\begin{proofsketch}
By observing the code, we know that from Line \ref{lin:remv2}, that when $LocateVertex(key)$ returns, vertex nodes $v_1$ and $v_2$ are locked, ($v_1, v_2$) $\in$ $\vnodes{S}$ and $v_1.val$ $<$ $key$ $\leq$ $v_2.val$. We know that the $\lp$ of this method is Line \ref{lin:remv3}, where the condition is evaluated to $false$. This means that $v_2.val$ $\neq$ $key$ such that $v_1.vnext = v_2$. Also since node values do not change after initialization. Hence $\vnode(key)$ $\notin$ $\pree{i}$.
\end{proofsketch}

\begin{lemma}
\label{lem:conVT-conc}
If some $\conv(key)$ method returns true in $E^H$, then the vertex node corresponding to that key must be present in the pre-state of \lp event of the method. Formally, \\ $\langle \conv(key, true) \Longrightarrow (\vnode(key) \in \pree{i} \rangle$. 
\end{lemma}

\begin{proofsketch}
By observing the code, we realise that at the end of while loop in Line \ref{lin:conv5} of $\conv(key)$ method, $v.val$ $\geq$ $key$. Also $v$ being a reference, does not change. To return true, $v.marked$ should be set to $false$ in the pre-state of $\lp$. It is clear that any unmarked public node should be reachable from $\vh$ and thereby belong to $S.\abgv$. We also know that a node's key value does not change after initialization. Hence $\vnode(key)$ $\in$ $\pree{i}$.
\end{proofsketch}

\begin{lemma}
\label{lem:conVF-conc}
If some $\conv(key)$ method returns false in $E^H$, then the vertex node corresponding to that key will not be present in the pre-state of \lp event of the method. Formally, \\ $\langle \conv(key, false) \Longrightarrow (\vnode(key) \notin \pree{i} \rangle$. 
\end{lemma}

\begin{proofsketch}
\begin{enumerate}
\item No successful concurrent $\addv$ on $key$: By observing the code, we realise that at the end of while loop at Line \ref{lin:conv5} of $\conv(key)$ method, $v.val$ $\geq$ $key$. Also $v$ being a reference, does not change. To return false, $v.marked$ should be set to true in the pre-state of $\lp$ in Line \ref{lin:conv6}. Since a node once marked, cannot be unmarked, therefore it does not belong to $S.\abgv$. Hence we conclude that, $\vnode(key)$ $\notin$ $\pree{i}$.
\item Concurrent successful $\addv(key)$ method: We know that the $\lp$ in this case is immediately before the LP of $\addv$ $\mth$. Also from Lemma \ref{lem:addVT-conc}, it follows that if $\addv(key)$ returns true, then the vertex node corresponding to that key is not present in the pre-state of the $\lp$. Hence we conclude that, $\vnode(key)$ $\notin$ $\pree{i}$.
\end{enumerate}
\end{proofsketch}

\begin{lemma}
\label{lem:addET-conc}
If some $\adde(key_1,key_2)$ method returns true in $E^H$, then the corresponding vertex nodes, $\vnode(key_1)$ and $\vnode(key_2)$ will be present in the pre-state of \lp event of the method. Formally, \\ $\langle \adde(key_1,key_2,true) \Longrightarrow (\vnode(key_1) \wedge \vnode(key_2)) \in \pree{i} \rangle$.
%as well as $\enode(key_2)$ may or may not present in the pre-state of the \lp event of the method,\\
%\begin{enumerate}
%\item $\langle \adde(key_1,key_2,true) \Longrightarrow (\vnode(key_1) \wedge \vnode(key_2) \wedge \enode(key_2)) \in \pree{i} \rangle$.
%\item  $\langle \adde(key_1,key_2,true) \Longrightarrow (\vnode(key_1) \wedge \vnode(key_2) \in \pree{i}) $ $\wedge (\enode(key_2) \notin \pree{i})\rangle$.
%\end{enumerate}
\end{lemma}

\begin{proofsketch}
\begin{enumerate}
\item No successful concurrent $\remv$ on $key_1$ \& $key_2$: By observing the code, we realise that $HelpSearchEdge$ returns successfully only when $\vnode(key_1)$ \& $\vnode(key_2)$ were found to be present in the vertex list at least in one state of the execution. Now after this, the vertex nodes are again tested for removal. Thus, we can conclude that in the post-state of Line \ref{lin:loce8:16}, vertex nodes $\vnode(key_1)$ and $\vnode(key_2)$ must belong to $S.\abgv$. Since there is no concurrent deletion of these vertices, we conclude that both the vertex nodes are present in the pre-state of $\lp$ of this method. Hence $(\vnode(key_1) \wedge \vnode(key_2))$ $\in$ $\pree{i}$.
    
\item Concurrent successful $\remv$ on $key_1$ or $key_2$ or both: We know that the $\lp$ in this case is immediately before the first $\lp$ of $\remv$ $\mth$. Also from Lemma \ref{lem:removeVT-conc}, it follows that if $\remv(key)$ returns true, then the vertex node corresponding to that key is present in the pre-state of the $\lp$. If any of the vertices were not present, the method returns $false$. Hence we conclude that, $(\vnode(key_1) \wedge \vnode(key_2))$ $\in$ $\pree{i}$.

%$ ((\vnode(key_1), \vnode(key_2))  \in \pree{i}  \wedge $ $(\enode(key_2) \in \pree{i} $: \\
%From Line \ref{lin:adde2}, when $LocateEdge(key_1, key_2)$ returns and we know that, vertex node $\vnode(key_1)$ and $\vnode(key_2)$ are in the $S.\abgv$, the edge nodes $e_1$ and $e_2$ are locked and ($e_1, e_2$) $\in$ $\enodes{S}$ and $e_1.val$ $<$ $key_2$ $\leq$ $e_2.val$. Now in Line \ref{lin:adde3}, $e_2.val$ $=$ $key_2$ is evaluated to $true$ such that $e_1.enext = e_2$ and $e_2$ $\in$ $\enodes{S}$ of the vertex $\vnode(key_1)$. We know $\enode(key_2)$ is belong to $S.\abge$ of the vertex $\vnode(key_1)$, where $S$ is the pre-state of the $LP$ event of the method. Hence $\enode(key_2)$ $\in$ $\pree{i}$.
\end{enumerate}
\end{proofsketch}


\begin{lemma}
\label{lem:addEF-conc}

If some $\adde(key_1,key_2)$ method returns false in $E^H$, then at least one of the vertex nodes corresponding to those keys will not be present in the pre-state of \lp event of the method. Formally, \\ $\langle$ $\adde((key_1,key_2), false) \Longrightarrow ((\vnode(key_1)$ $\vee$ $(\vnode(key_2)) \notin \pree{i} \rangle$. 

%If some $\adde(key_1, key_2)$ method returns false with no successful concurrent \addv in $E$ then ($vnode(key_1)$ \text{ OR } $vnode(key_1)$) $\notin$ $S.\abgv$ where $S$ is the pre-state of LP event of the method.
\end{lemma}

\begin{proofsketch}

\begin{enumerate}
\item No successful concurrent $\addv$ on $key_1$ and $key_2$:
 By observing the code, we realise that in the Line \ref{lin:helploce8}/\ref{lin:helploce8.1} vertex node $\vnode(key_1)$ $\notin$ $S.\abgv$ because it is not reachable from $\vh$ or marked. Also, in the Line \ref{lin:helploce16}/\ref{lin:helploce16.1} vertex node $\vnode(key_2)$ $\notin$ $S.\abgv$ because it is not reachable from $\vh$ or marked. Consequently, the Line \ref{lin:loce8:16} returns $false$, if $read(v_1.marked)$ or $read(v_2.marked)$ is set depending upon the execution. Hence, $\langle (\vnode(key_1)$ $\vee$ $(\vnode(key_2)$) $\notin$ $\pree{i} \rangle$.
\item Concurrent successful $\addv$ on $key_1$ or $key_2$ or both: We know that the $\lp$ in this case is immediately before the first $\lp$ of $\addv$ $\mth$ on $u$ and $v$. Also from Lemma \ref{lem:addVT-conc}, it follows that if $\addv(key)$ returns true, then the vertex node corresponding to that key is not present in the pre-state of the $\lp$. Hence we conclude that, $\langle (\vnode(key_1)$ $\vee$ $(\vnode(key_2)$) $\notin$ $\pree{i} \rangle$.
\end{enumerate}
\end{proofsketch}

\begin{lemma}
\label{lem:removeET-conc}
If some $\reme(key_1,key_2)$ method returns true in $E^H$, then the corresponding vertex nodes, $\vnode(key_1)$ and $\vnode(key_2)$ must be present in the pre-state of \lp event of the method Formally, \\
%\begin{enumerate}
$\langle \reme(key_1,key_2,true) \Longrightarrow (\vnode(key_1) \wedge \vnode(key_2)) \in \pree{i} \rangle$.
%\item  $\langle \reme(key_1,key_2,true) \Longrightarrow ((\vnode(key_1)) \wedge (\vnode(key_2) )\in \pree{i}$ $\wedge \enode(key_2)) \notin \pree{i}) \rangle$.
%\end{enumerate}
\end{lemma}

\begin{proofsketch}
Similar argument as Lemma \ref{lem:addET-conc}.
%\begin{enumerate}
%\item ($(\vnode(key_1), \vnode(key_2))  \in \pree{i}) \wedge  $ $(\enode(key_2) \in \pree{i})$:\\
%\begin{enumerate}
%\item No successful concurrent $\remv$ on $key_1$ and $key_2$: From Line \ref{lin:reme2}, when $LocateEdge(key_1, key_2)$ returns with no successful concurrent $\remv$ we know that, vertex node $\vnode(key_1)$ and $\vnode(key_2)$ are in the $\vnodes{S}$, edge node $e_1$ and $e_2$ are locked,  ($e_1, e_2$) $\in$ $\enodes{S}$ and $e_1.val$ $<$ $key_2$ $\leq$ $e_2.val$. Now in Line \ref{lin:reme3}, $e_2.val$ $=$ $key_2$ is evaluated to $true$ such that $e_1.enext = e_2$ and $e_2$ $\in$ $\enodes{S}$ of the vertex $\vnode(key_1)$. The $\enode(key_2)$ is belong to $S.\abge$ of the vertex $\vnode(key_1)$. Hence, ( $(\vnode(key_2),\vnode(key_1))  \wedge (\enode(key_2)$ $\in$ $\pree{i}$.
%\item Successful concurrent $\remv$ on $u$ or $v$: 
%We know that the $\lp$ in this case is immediately before the first $\lp$ of $\remv$ $\mth$. Also from Lemma \ref{lem:removeVT-conc}, it follows that if $\remv(key)$ returns $true$, then the vertex node corresponding to that key is present in the pre-state of the $\lp$. Hence we conclude that, $(\vnode(key_1) \wedge \vnode(key_2))$ $\in$ $\pree{i}$.    
%\end{enumerate}


%\item $((\vnode(key_1), \vnode(key_2))  \in \pree{i} ) \wedge $ $(\enode(key_2) \notin \pree{i}) $: \\
%\end{enumerate}

\end{proofsketch}

\begin{lemma}
\label{lem:removeEF-conc}
If some $\reme(key_1,key_2)$ method returns false in $E^H$, then at least one of the vertex nodes, $\vnode(key_1)$ and $\vnode(key_2)$ will be not present in the pre-state of \lp event of the method. Formally, $\langle \reme(key_1,key_2, false) \Longrightarrow (\vnode(key_1) \vee \vnode(key_2) ) \notin \pree{i} \rangle$.
\end{lemma}

\begin{proofsketch}
Similar argument as Lemma \ref{lem:addEF-conc}.
 %From Line \ref{lin:reme2}, when $LocateEdge(key_1, key_2)$ returns we know that, vertex node $\vnode(key_1)$ or $\vnode(key_2)$ may not in the $S.\abgv$. In the Line \ref{lin:helploce8}/ \ref{lin:helploce8.1} vertex node $\vnode(key_1)$ $\notin$ $S.\abgv$ or it is marked and in the Line \ref{lin:helploce16}/ \ref{lin:helploce16.1} vertex node $\vnode(key_2)$ $\notin$ $S.\abgv$ or it is marked. So ($\vnode(key_1)$ \text{ OR } $\vnode(key_1)$) $\notin$ $S.\abgv$ where $S$ is the pre-state of LP event of the method. Hence, $\langle \reme((key_1,key_2), false) \Longrightarrow ((\vnode(key_1) OR (\vnode(key_2)) \notin \pree{i} \rangle$.
\end{proofsketch}


\begin{lemma}
\label{lem:conET-conc}
If some $\cone(key_1, key_2)$ method returns true in $E^H$, then both the vertex nodes, $\vnode(key_1)$ \& $\vnode(key_2)$ and the edge node corresponding to it, $\enode(key_2)$ must be present in the pre-state of \lp event of the method. Formally, \\ $\langle \cone(key_1, key_2, true) \Longrightarrow (\vnode(key_1) \wedge \vnode(key_2) \wedge \enode(key_2))\in \pree{i} \rangle$. 
\end{lemma}

\begin{proofsketch}
\begin{enumerate}
\item No successful concurrent $\remv$ on $key_1$ and $key_2$ and no successful $\reme(key_1,key_2)$: By observing the code, we realise that $HelpSearchEdge$ returns successfully only when $\vnode(key_1)$ \& $\vnode(key_2)$ were found to be present in the vertex list at least in one state of the execution. Thus, we can conclude that in the post-state of Line \ref{lin:cone16}, vertex nodes $\vnode(key_1)$ and $\vnode(key_2)$ belong to $S.\abgv$ (since there is no concurrent $\remv$). Now in the end of the Line \ref{lin:cone17.1}, $key_2$ $\leq$ $e.val$. Now in Line \ref{lin:cont-tf:Edge}, $e.val$ $=$ $key_2$ is evaluated to $true$. Also $e$ being a reference, does not change. It is clear that any unmarked public node should be reachable from $\vh$ and thereby belong to $S.\abge$. $\langle (\vnode(key_1) \wedge \vnode(key_2) \wedge \enode(key_2))\in \pree{i} \rangle$. 

\item Successful concurrent $\remv$ on $key_1$ or $key_2$ or Successful $\reme(key_1,key_2)$: We know that the $\lp$ in this case is immediately before the first $\lp$ of $\remv$ $\mth$ on $\vnode(key_1)$ and $\vnode(key_2)$ and $\reme$ of $\enode((key_1,key_2))$. Also from Lemma \ref{lem:removeVT-conc}, it follows that if $\remv(key_1)$ or $\remv(key_2)$ returns true, then the vertex node corresponding to that key is present in the pre-state of the $\lp$. Also from Lemma \ref{lem:removeET-conc}, it follows that if $\reme(key_1, key_2)$ returns true, then the edge node $\enode(key_2)$ corresponding to that key is present in the pre-state of the $\lp$. Hence we conclude that, $\langle (\vnode(key_1) \wedge \vnode(key_2) \wedge \enode(key_2))\in \pree{i} \rangle$. 
\end{enumerate}
\end{proofsketch}

\begin{lemma}
\label{lem:conEF-conc}
If some $\cone(key_1, key_2)$ method returns false in $E^H$, then the edge node corresponding to it, $\enode(key_2)$ will not be present in the pre-state of \lp event of the method. Formally, \\ $\langle \cone(key_1, key_2, false) \Longrightarrow \enode(key_2) \notin \pree{i} \rangle$. 
\end{lemma}

\begin{proofsketch}


\begin{enumerate}
\item No successful concurrent $\adde$ on $(key_1, key_2)$: By observing the code, we realise that in the Line \ref{lin:helploce8}/\ref{lin:helploce8.1} vertex node $\vnode(key_1)$ $\notin$ $S.\abgv$ because it is not reachable from $\vh$ or marked. Also, in the Line \ref{lin:helploce16}/\ref{lin:helploce16.1} vertex node $\vnode(key_2)$ $\notin$ $S.\abgv$ because it is not reachable from $\vh$ or marked, depending upon the execution. Therefore, $(\vnode(key_1)$ $\vee$ $(\vnode(key_2)$) $\notin$ $S.\abgv$. This implies that from the case $1$ of Lemma \ref{lem:addEF-conc}. Hence $\langle \enode(key_2) \notin \pree{i} \rangle$.

\item Concurrent successful $\adde(key_1, key_2)$ : We know that the $\lp$ in this case is immediately before the first $\lp$ of $\adde$ $\mth$ on  $(key_1, key_2)$. Also from Lemma \ref{lem:addET-conc}, it follows that if $\adde(key_1, key_2)$ returns true, then the vertex node corresponding to that key is not present in the pre-state of the $\lp$.  Hence $\langle \enode(key_2) \notin \pree{i} \rangle$.


\end{enumerate}
\end{proofsketch}

\ignore{
\begin{observation}
	\label{obs:node-marknext:vertex}
Consider a global state $S$ which has a node $n$ which is marked. Then in any future state $S'$ $n.vnext$ remains unchanged. Formally, $\langle \forall S, S': (n \in S.vnodes) \land (S.n.marked) \land (S \sqsubset S') \Longrightarrow (S'.n.vnext = S.n.vnext) \rangle$. \qed

\end{observation}

\begin{observation}
\label{obs:consec-next:vertex}
In any global state $S$ which has two non-consecutive $VNode$s $n_p$, $n_q$ where $n_p$ is unmarked and $n_q$ is marked, then in any future state $S'$, $n_p$ cannot point to $n_q$. Formally, $\langle \neg (S.n_p.marked) \land (S.n_q.marked) \land (S.n_p.next \neq n_q) \land (S \sqsubset S') \Longrightarrow (S'.n_p.next \neq S'.n_q) \rangle$. \qed
\end{observation}

\begin{lemma}
\label{lem:consec-mark:vertex}
Consider a global state $S$ which has two consecutive nodes $n_p$, $n_q$ which are marked. Then we say that marking event of $n_p$ happened before marking event of $n_q$. Formally, $\langle \forall S: (n_p, n_q \in S.nodes) \land (S.c_p.marked) \land (S.c_q.marked) \land (S.c_p.next = S.c_q) \Rightarrow (c_p.marked <_E c_q.marked) \rangle$.
\end{lemma}

\begin{proofsketch}
\begin{figure}[tbph]
\centerline{\scalebox{0.6}{\input{figs/lemma26.pdf_t}}}
\caption{LP of $contains(key, false)$ is at $read(c.val$ = $key)$ at Line 6}
%\label{fig:trans-tree}
\end{figure}

We prove by contradiction. Assume that in some state $S'$ immediately after marking $c_q$, $c_q$ was marked before $c_p$. So we know that in $S'$, $c_p$ is unmarked and $c_q$ is marked. Let us also assume that in $S'$, $c_p.next$ $\neq$ $c_q$. So, $S'.c_p.next$ $\neq$ $S'.c_q$ $\land \neg S'.c_p.marked$. Also in the state $S$, we have that $S.c_p.next = S.c_q$ and $c_p$ and $c_q$ are both marked. This contradicts our Observation \ref{obs:consec-next:vertex} that $S'.c_p.next$ $\neq$ $S'.c_q$. Hence in $S'.c_p.next = S'.c_q$.
Consider some state $S''$ immediately before marking event of $c_q$. We know that $S''.c_p.next = S''.c_q$ (from Observation \ref{Obs:locate:vertex}  $pred$ and $curr$ locked) and $c_p$, $c_q$ are both unmarked. Then in some state $R$ after $S'$ and before $S$, $R.c_p.next$ $\neq$ $R.c_q$. From Observation \ref{obs:consec-next:vertex}, unmarked node cannot point to marked node. Hence in state $S$ also, we will have that $S.c_p.next$ $\neq$ $S.c_q$. This contradicts our given statement that $S.c_p.next = S.c_q$. Hence proved that in $S'$, $c_p$ was marked before $c_q$.

\end{proofsketch}

}




\begin{lemma}
\label{lem:pre-ret}
$\langle  \pree{i} = \prem{i} 
\Longrightarrow  \rete{i} = \retm{i} \rangle$
\end{lemma}

\begin{proofsketch}

\noindent We prove by Induction on $\lp$ events,\\[0.1cm]
\textbf{Base Step:} Initially, we know that after the first $\lp$ event the return values will be same in both $E^H$ and $E^S$.\\[0.1cm]
\textbf{Induction Hypothesis:} \\[0.1cm]
We assume that $k^{th}$ event corresponding to the $k^{th}$ method is $\lp$ and $\pree{k} = \prem{k}$ $\Longrightarrow$ $\rete{k} = \retm{k} $ \\[0.3cm]
\textbf{Induction Step:} \\
We need to prove that $(k+1)^{th}$ event corresponding to the $(k+1)^{th}$ method satisfies: $\pree{k+1} = \prem{k+1}$ $\Longrightarrow$ $\rete{k+1} = \retm{k+1}$ \\[0.2cm]
We know from Lemma \ref{lem:conce-seqe-mi} that,\\ 
$(\pree{i} = \prem{i})\Longrightarrow (\poste{i} = \postm{i})$\\[0.2cm]
Now to prove that the return values are same, we have the following cases that $(k+1)^{th}$ event is $\lp$ of either of these methods:

\begin{enumerate}
\item \textbf{\addv Method:}
\begin{itemize}
\item \textbf{Return true}: We need to prove that $\vnode(key)$ $\notin$ $\pree{i}$, which follows from Lemma \ref{lem:addVT-conc}. We know that if $\vnode(key)$ $\notin$ the pre-state of $\lp$ of $\addv$ method, then the $\addv$ method must return $true$ in $E^S$.

%\item \textbf{Return false}, then $\lp$ is the read at Line \ref{lin:addv3} of $\addv$ method. We need to prove that \textit{\vnode(key)} $\in$ $\pree{i}$, which follows from Lemma \ref{lem:addF-conc}. We know that if $\vnode(key)$ $\in$ pre-state of $\lp$ of $\addv$ method, then the $\addv$ method must return false in $E^S$.
\end{itemize}

\item \textbf{\remv Method:}
\begin{itemize}
\item \textbf{Returns true}: We need to prove that $\vnode(key)$ $\in$ $\pree{i}$, which follows from Lemma \ref{lem:removeVT-conc}. We know that if $\vnode(key)$ $\in$ pre-state of $\lp$ of $\remv$ method, then the $\remv$ method must return true in $E^S$.

\item \textbf{Returns false}: We need to prove that $\vnode(key)$ $\notin$ $\pree{i}$, which follows from Lemma \ref{lem:removeVF-conc}. We know that if $\vnode(key)$ $\notin$ pre-state of $\lp$ of $\remv$ method, then the $\remv$ method must return false in $E^S$.
\end{itemize}

\item \textbf{\conv Method:}
\begin{itemize}
\item \textbf{Returns true}: We need to prove that $\vnode(key)$ $\in$ $\pree{i}$, which follows from Lemma \ref{lem:conVT-conc}. We know that if $\vnode(key)$ $\in$ pre-state of $\lp$ of $\conv$ method, then the $\conv$ method must return $true$ in $E^S$.\\
 
\item \textbf{Returns false}: We need to prove that $\vnode(key)$ $\notin$ $\pree{i}$, which follows from Lemma \ref{lem:conVF-conc}. We know that if $\vnode(key)$ $\notin$ pre-state of $\lp$ of $\conv$ method, then the $\conv$ method must return $false$ in $E^S$. \qed

\end{itemize}

\item \textbf{\adde Method:}
\begin{itemize}
\item \textbf{Return true}: We need to prove that $(\vnode(key_1)\wedge \vnode(key_2))$ $\in$ $\pree{i}$, which follows from Lemma \ref{lem:addET-conc}. We know that if $\vnode(key_1)$ and $\vnode(key_2)$ are present in the pre-state of $\lp$ of $\adde$ method, then the $\adde$ method must return $true$ in $E^S$.

\item \textbf{Return false}: 
We need to prove that $(\vnode(key_1)\vee \vnode(key_2))$ $\notin$ $\pree{i}$, which follows from Lemma \ref{lem:addEF-conc}. We know that if $\vnode(key_1)$ or $\vnode(key_2)$ is not present in the pre-state of $\lp$ of $\adde$ method, then the $\adde$ method must return $false$ in $E^S$.

\end{itemize}
\item \textbf{\reme Method:}
\begin{itemize}
\item \textbf{Returns true}: 
We need to prove that $(\vnode(key_1)\wedge \vnode(key_2))$ $\in$ $\pree{i}$, which follows from Lemma \ref{lem:removeET-conc}. We know that if $\vnode(key_1)$ and $\vnode(key_2)$ are present in the pre-state of $\lp$ of $\reme$ method, then the $\reme$ method must return $true$ in $E^S$.


\item \textbf{Returns false}: 
We need to prove that $(\vnode(key_1)\vee \vnode(key_2))$ $\notin$ $\pree{i}$, which follows from Lemma \ref{lem:removeEF-conc}. We know that if $\vnode(key_1)$ or $\vnode(key_2)$ is not present in the pre-state of $\lp$ of $\reme$ method, then the $\reme$ method must return $false$ in $E^S$.

\end{itemize}

\item \textbf{\cone Method:}
\begin{itemize}

\item \textbf{Returns true}:

We need to prove that $(\vnode(key_1) \wedge \vnode(key_2) \wedge \enode(key_2))\in \pree{i}$, which follows from Lemma \ref{lem:conET-conc}. We know that if $\vnode(key_1)$ and $\vnode(key_2)$ and $\enode(key_2)$ are present in the pre-state of $\lp$ of $\cone$ method, then the $\cone$ method must return $true$ in $E^S$.


\item \textbf{Returns false}: 
We need to prove that $\enode(key_2)$ $\notin$ $\pree{i}$, which follows from Lemma \ref{lem:conEF-conc}. We know that if $\enode(key_2)$ is not present in the pre-state of $\lp$ of $\cone$ method, then the $\cone$ method must return $false$ in $E^S$.

\end{itemize}
\end{enumerate}

\end{proofsketch}

\begin{lemma}
\label{lem:ret-lin}
$ \rete{i} = \retm{i} \Longrightarrow$ $H$ is Linearizable.
\end{lemma}

\begin{proofsketch}
By the definition of Linearizability.
\end{proofsketch}

\begin{lemma}
\label{lem:hist-lin}
Every history $H$ generated by the interleaving of any of the methods of the concurrent graph data structure, is linearizable.
\end{lemma}

\begin{proofsketch}
This can be derived by combining Lemma \ref{lem:conce-seqe-pre}, \ref{lem:pre-ret} \& \ref{lem:ret-lin}.
\end{proofsketch}
}

\ignore{
\subsection{Safety: Proof Skeleton}

\noindent In this subsection, we describe the lemmas to prove the correctness of our \cgds.

\begin{observation}
\label{obs:change-abs}
	Only the \lp events in the execution can change the \abg. \qed
\end{observation}

\begin{lemma}
\label{lem:seqe-pre}
The global state of the graph after the \rsp event of a method is the same as the state before the \inv event of the consecutive method in the sequential execution. Formally, $\langle \postm{i}= \prem{i+1}\rangle$
\end{lemma}

\begin{proofsketch}
From the definition of Sequential Execution as depicted in Figure \ref{fig:conc:seq}(b).
\end{proofsketch}

\begin{lemma}
\label{lem:conce-pre}
In every concurrent execution ordered by its events, the global state of the graph immediately after a \lp event is the same as the state before the next \lp event. Formally, $ \langle \poste{i} = \pree{i+1} \rangle$
\end{lemma}

\begin{proofsketch}
\ignore{Let us prove by contradiction. Assume that there exists a method $m_k$ which modifies the $\abg$ between method $m_i$ and $m_{i+1}$.
As we know from the code that the events $write(v_1.vnext, v_3)$ in Line \ref{lin:addv6} of $\addv$,  $write(v_2.marked, true)$ in Line \ref{lin:remv4} of $\remv$, $write(e_1.enext, e_3)$ in Line \ref{lin:adde6} of $\adde$ and $write(e_2.marked, true)$ \ref{lin:reme4} of $\reme$ method can change the $\abg$ only. Any other events between the post-state of $E.m_i.\lp$ and the pre-state of $E.m_{i+1}.\lp$ will not change the $\abg$. Hence Proved.} From Observation \ref{obs:change-abs} as illustrated by Figure \ref{fig:conc:seq}(a).
\end{proofsketch}

%\ignore{
\begin{lemma}
\label{lem:conce-seqe-mi}

Consider a concurrent history $H$ and a sequential history $S$. Let $m_x, m_y$ be \mth{s} in $H$ and $S$ respectively. Suppose the following are true (1) The \abg in the pre-state of $m_x$'s \lp in $H$ is the same as the \abg in the pre-state of $m_y$ in $S$;  (2) The \inv events of $m_x$ and $m_y$ are the same. Then (1) the $\rsp$ event of $m_x$ in $H$ must be same as $\rsp$ event of $m_y$ in $S$; (2) The \abg in the post-state of $m_x$'s \lp in $H$ must be the same as the \abg in the post-state of $m_y$ in $S$. Formally, $\langle \forall m_x \in E^H, \forall m_y \in E^S: (\prees{m_x} = \prems{m_y}) \wedge (\inves{m_x} = \invms{m_y}) \Longrightarrow (\postes{m_x} = \postms{m_y}) \wedge (\retes{m_x} = \retms{m_y}) \rangle$.
\end{lemma}
\ignore{
If the pre-state of a \lp event in the concurrent execution is the same as the pre-state of a method in sequential execution, then the post-state of the \lp event in concurrent execution must be same as the post-state of the method in sequential execution. Formally,
$ \langle(\pree{i} = \prem{i})\Longrightarrow (\poste{i} = \postm{i}) \rangle$.
}


\begin{proofsketch}
From Observation \ref{obs:change-abs}, we know that there is only one event which can change $AbG$ i.e. $\lp$. Given that the pre-states are same, only $\lp$ event gets executed in the execution (which is an atomic event), then on execution in sequential and concurrent execution, post-state remains same.
\end{proofsketch}

\begin{lemma}
\label{lem:conce-seqe-pre}
In every execution, the pre-state of \lp event must be same as the pre-state of the method in the sequential execution. Formally,
$\langle \pree{i} = \prem{i} \rangle$.
\end{lemma}

\ignore{
\begin{proofsketch}
We prove by Induction on events which are the linearization points of the methods,\\[0.1cm]
\textbf{Base Step:} Before the $1^{st}$ $\lp$ event, the initial $\abg$ remains same because all the events in the concurrent execution before the $1^{st}$ $\lp$ do not change $\abg$.\\[0.3cm]
\textbf{Induction Hypothesis}: Let us assume that the first $k$ $\lp$ events, we know that,\\[0.2cm]  
$\pree{k} = \prem{k}$ \\[0.3cm]
\textbf{Induction Step:} We have to prove that: $\pree{k+1} = \prem{k+1}$ holds true.\\[0.3cm]
We know from Induction Hypothesis that for $k^{th}$ method,\\[0.3cm]
$\pree{k} = \prem{k}$\\[0.3cm]
Now we know $\lp$ is an atomic event that is same in $E^H$ and $E^S$. From the Lemma \ref{lem:conce-seqe-mi} we have,
\begin{equation} 
\begin{split}
\label{lab:eq:conce-seqe-mi}
 (\pree{k} = \prem{k}) \xRightarrow[]{\text{From Lemma \ref{lem:conce-seqe-mi}}}\\ (\poste{k} = \postm{k})
 \end{split}
\end{equation} 

From the Lemma \ref{lem:seqe-pre}, we have,

\begin{equation} 
\label{lab:eq:seqe-pre}
 \postm{k} \xRightarrow[]{\text{From Lemma \ref{lem:seqe-pre}}}  \prem{k+1} 
\end{equation} 

From the equation \ref{lab:eq:conce-seqe-mi}
we have,
\begin{equation} 
\label{lab:eq:seqe-mi-post}
 \poste{k} =  \postm{k}
\end{equation} 

By combining the equation \ref{lab:eq:seqe-mi-post} and \ref{lab:eq:seqe-pre} we have,

\begin{equation} 
\label{lab:eq:seqe-mi-pre}
 \poste{k} =  \prem{k+1}
\end{equation} 

And from the Lemma \ref{lem:conce-pre} we have, \begin{equation} 
\label{lab:eq:conce-pre}
 \poste{k} =  \pree{k+1}
\end{equation}

So, by combining equations \ref{lab:eq:conce-pre} and \ref{lab:eq:seqe-mi-pre} we get,

\begin{equation} 
\label{lab:eq:conce-seuq-pre}
 \pree{k+1} =  \prem{k+1}
\end{equation}

Finally, $\pree{k+1} = \prem{k+1}$.\\[0.3cm]
Hence this holds for all $m_i$ in $E^H$. Hence Proved.

\end{proofsketch}
}

\begin{lemma}
\label{lem:pre-ret}
For any \mth $m_i$ in $H, S$ the \abg in the pre-state of the \lp of $m_i$ in $H$ is the same as the \abg in the pre-state of $m_i$ in $S$. Formally, $\langle  \pree{i} = \prem{i} \Longrightarrow  \rete{i} = \retm{i} \rangle$
\end{lemma}

\begin{lemma}
\label{lem:ret-lin}
The return values for all the \mth{s} in $H$ \& $S$ are the same. Formally, $ \rete{i} = \retm{i} \Longrightarrow$ $H$ is Linearizable.
\end{lemma}

\begin{proofsketch}
By the definition of Linearizability.
\end{proofsketch}

\begin{lemma}
\label{lem:hist-lin}
Every history $H$ generated by the interleaving of any of the methods of the concurrent graph data structure, is linearizable.
\end{lemma}

\begin{proofsketch}
This can be derived by combining Lemma \ref{lem:conce-seqe-pre}, \ref{lem:pre-ret} \& \ref{lem:ret-lin}.
\end{proofsketch}


\subsection{Liveness: Proof Outline}
In this subsection we prove the progress guarantee of the methods of our proposed graph data structure. 
}
\vspace{-3mm}
\begin{lemma}
\label{lem:linealizability}
	The algorithms employed for our \cgds are linearizable.
\end{lemma}

\begin{lemma}
\label{lem:prog:add:rem}
	The methods $\addv$, $\remv$, $\adde$ and $\reme$ are deadlock-free and $\conv$ and $\cone$ are wait-free.
\end{lemma}
\ignore{
\begin{proofsketch}
\noindent
We prove all the $\addv$, $\remv$, $\adde$ and $\reme$ methods are deadlock-free by direct argument based of the acquiring lock on both the current and predecessor nodes.
\begin{enumerate}
    \item $\addv$: the $\addv(key)$ method is deadlock-free because a thread always acquires lock on the $\vnode$ with larger keys first. Which means, if a thread say $T_1$ acquired a lock on a $\vnode(key)$, it never tries to acquire a lock on a $\vnode$ with key greater than or equal to $\vnode(key)$. This is true because the $\addv$ method acquires lock on the predecessor $\vnode$ from the $LocateVertex$ method. This $LocateVertex$ method returns $\langle v_1, v_2 \rangle$, both the vertex nodes $v_1$ and $v_2$ are locked, $v_1$ and $v_2$ are not marked and $v_1.vnext$ = $v_2$. 
    \item $\remv$: the $\remv(key)$ method is also deadlock-free, similar argument as $\addv$. 
    \item $\adde$: the $\adde(key_1, hey_2)$ method is deadlock-free because a thread always acquires lock on the $\enode$ with lager keys first. Which means, if a thread say $T_1$ acquired a lock on a $\enode(key_2)$, it never tries to acquire a lock on a $\enode$ of the vertex $\vnode(key_1)$ with key greater than or equal to $\enode(key_2)$. This is true because the $\adde$ method acquires lock on the predecessor edge nodes of the vertex $\vnode(key_1)$ from the $LocateEdge$ method. This $LocateEdge$ method returns $\langle e_1, e_2 \rangle$, both the $\enode$ of the vertex $\vnode(key_1)$ $e_1$ and $e_2$ are locked, $e_1$ and $e_2$ are not marked and $e_1.enext$ = $e_2$. 
    \item $\reme$: the $\reme(key_1, key_2)$ method is also deadlock-free, similar argument as $\adde$. 
\end{enumerate}

\end{proofsketch}

\begin{lemma}
\label{lem:prog:con}
	The methods $\conv$ and $\cone$ are wait-free.
\end{lemma}


\begin{proofsketch}
\noindent
The $\conv(key)$ method scans the vertex list of the graph starting from the $\vh$, ignoring whether $\vnode$ are marked or not. It returns a boolean $flag$ either $true$ or $false$ depending on $\vnode(key)$ greater than or equal to the sought-after key. If the desired $\vnode$ is unmarked, it simply returns $true$ and this is correct because the vertex list is sorted. On the other hand, it returns $false$ if $\vnode(key)$ is not present or has been marked. This $\conv$ method is wait-free, because there are only a finite number of vertex keys that are smaller than the one being searched for. By the observation of the code, a new $\vnode$ with lower or equal keys is never added ahead of it, hence they are reachable from $\vh$ even if vertex nodes are logically removed from the vertex list. Therefore, each time the  $\conv$ moves to a new vertex node, whose key value is larger key than the previous one. This can happen only finitely many times, which says the traversal of $\conv$ method is wait-free.

Similarly, the $\cone(key_1, key_2)$ method first scans the vertex list of the graph starting from the $\vh$, ignoring whether vertex nodes are marked or not. It returns a boolean $flag$ either $true$ or $false$ depending on $\enode(key_2)$ greater than or equal to the sought-after key in the edge list of the vertex $\vnode(key_1)$. If the desired $\enode$ is unmarked, it simply returns $true$ and this is correct because the vertex list is sorted as well as the edge list of the vertex $\vnode(key_1)$ is also sorted. On the other hand it returns $false$ if either $\vnode(key_1)$ or $\vnode(key_2)$ is not present or has been marked in the vertex list or $\enode(key_2)$ is not present or has been marked in the edge list of the vertex $\vnode(key_1)$. This $\cone$ method is wait-free, because there are only a finite number of vertex keys that are smaller than the one being searched for as well as a finite number of edge keys that are smaller than the one being searched for in edge list of any vertex . By observation of the code a new $\enode$ with lower or equal keys is never added ahead of $\enode(key_2)$ in the edge list of the vertex $\vnode(key_1)$, hence they are reachable from $\vh$ even if vertex nodes or edge nodes of $\vnode(key_1)$ are logically removed from the vertex list. Therefore, each time the  $\cone$ moves to a new edge node, whose key value is larger key than the previous one. This can happen only finitely many times, which says the traversal of $\cone$ method is wait-free. 
\end{proofsketch}
 
 }
 

==> dec_scc.tex <==
\section{Decremental Maintenance of Strongly Connected Component}
\label{sec:decscc}

==> full_scc.tex <==
\section{Fully Dynamic Maintenance of Strongly Connected Component}
\label{sec:fullscc}

==> inc_scc.tex <==
\section{Incremental Maintenance of Strongly Connected Component}
\label{sec:incscc}

==> related-work.tex <==
\section{Related Work}
\label{sec:related-work}
It can be seen that the graph acyclic problem gets complicated if the graph is huge and multiple threads are concurrently accessing the graph and performing some operations. There are many efficient well-known algorithms for solving these problems in the sequential world. However, there are a very few works in the area of concurrent graphs shared memory setting. There has been a recent and relevant work on the area of concurrent graphs by Kallimanis and Kanellou \cite{Kallimanis}. Their work also discusses about concurrent graph which supports operations; addition/deletion of edges and dynamic traversal. But they represent dynamic graph in the form of adjacency matrix with fixed upper-limit on the total number of vertices. Hence, their work can not be used to build \sgt scheduler. Moreover, it is not obvious how to extend their work to check for graph acyclicity.

==> result.tex <==
\section{Simulation Results \& Analysis}
\label{sec:simulation-results}
%--------------------------------------
\ignore{
\begin{figure*}[h]
\centering
  \begin{tabular}{@{}cccc@{}}
    \includegraphics[width=.32\textwidth]{figs/res1} &
    \includegraphics[width=.32\textwidth]{figs/res2} &
    \includegraphics[width=.32\textwidth]{figs/res3}
    \\
 a) & b) & c) \\
   \end{tabular}
  \captionof{figure}{a) Speedup obtained against sequential v/s Number of operations/thread for \textit{Contains-dominated} workload b) \textit{Update-dominated} workload c) \textit{Acyclicity Data Structure} }
\label{results}
\end{figure*}

}
%-------------------------------------
\vspace{-2mm}
\noindent We performed our tests on 2 sockets \& 14 cores per socket Intel Xeon (R) CPU E5-2660 v4 running at 2.00 GHz core frequency. Each core supports 2 hardware threads. Every core's L1, L2 cache are private to that core; L3 cache (35MB) is shared across all cores of a processors. The tests were performed in a controlled environment, where we were the sole users of the system. The implementation was written in C++ and threading is achieved by using Posix threads. The complete source code is available at \cite{Pdcrl-ConcurrentGraphDS2017}. \\[0.15cm]
In the experiments conducted, we start with an initial complete acyclic graph. When the program starts, it creates threads and each thread randomly performs a set of operations chosen by a particular workload distribution. Here, the evaluation metric used is the time taken to complete all the operations. We measure throughput obtained on running the experiment for 20 seconds and present the results for the following workload distributions: (a) \textit{Update-dominated}: $25\%$ $\addv$, $25\%$ $\adde$, $10\%$  $\remv$, $10\%$  $\reme$, $15\%$  $\conv$ and $15\%$  $\cone$ (b) \textit{Contains-dominated}:$40\%$  $\conv$, $40\%$  $\cone$, $7\%$ $\addv$, $7\%$ $\adde$, $3\%$  $\remv$ and $3\%$  $\reme$ (c) $50\%$ $\adde$, $50\%$  $\reme$ and rest are $0\%$,  the performance results are depicted in Figure (d), (e) and (f). Each data point is obtained after averaging for 5 iterations. Assume: no garbage collection and duplicate vertices are not inserted.


%\vspace{-0.4cm}



%\vspace{-0.4cm}

\noindent We tested different variants of the data structure - VElock-NoDIE: the concurrent data structure presented without Deletion of Incoming Edges (DIE) for deleted vertices, VElock-DIE: supporting Deletion of Incoming Edges of deleted vertices, CoarseLock: which supports concurrent operations by acquiring a global lock. The Figure (a), (b) and (c) depicts the performance results for the increasing number of thread (following a workload distribution) on the concurrent graph data structure. It can be seen that a significant speedup is obtained for the fine grained lock implementation. Figure \ref{fig:acyclic:ds} portrays the results of the graph acyclicity data structure with 25\% $\acadde$ calls. The cycle detection method has been implemented via reachability methods as described in the Section \ref{sec:Maintaining-Graph-Acyclicity}. These are compared against a coarse lock implementation of the incremental cycle detection method. The results depict that update \mth{s} with reachability based cycle detection (without deletion of incoming edges) gives a significant speedup and scales well with the increasing number of operations. 


==> scc.tex <==


\section{Strongly Connected Components(SCC)}
\label{sec:ssc}



\subsection{Non-blocking SGT Methods}



It takes a directed graph with n vertices and m edges as input.
The algorithm handles the following operations:

SCC(u,v): Checks if u and v are in the same SCC.
	Process: Checks if there is a directed path from u to v and if there is a directed path  from v to u.


A graph is strongly connected if there is a \emph{directed path} from any vertex to every other vertex. Formally, \\
Let $G=(V, E)$ be a directed graph. We say two nodes $u, v \in V $ are called  strongly  connected  iff  $v$ is reachable from $u$ and also $u$ is reachable from  $v$. A strongly connected component(or SCC) of $G$ is a set $C \subseteq V$ such that: 
 \begin{enumerate}
 \item $C$  is not empty.
 \item For any  $u, v \in C$: $u$ and $v$ are strongly connected.
 \item For any $u \in C$ and $v \in V-C$: $u$ and $v$ are not strongly connected.
 \end{enumerate}
\noindent 
 Also SCC is an equivalence relation on the set of vertices:
\begin{enumerate}
\item \textbf{Reflexive:} Every vertex $v$ is strongly connected to itself.
\item \textbf{Symmetric:} If $u$ is strongly connected to $v$, then $v$ is strongly connected to $u$.
\item \textbf{Transitive:} If $u$ is strongly connected to $v$ and $v$ is strongly connected to $w$, then $u$ is also strongly connected to $w$. 
\end{enumerate}

\noindent \textbf{Abstract class of SCC}
 \begin{verbatim}
 class SCC{
   list allSCC(); // returns all SCC list
   int countSCC(); //counts the number of strong connected components.
   boolean checkSCC(u,v); // whether u and v are connected 
   int blongsTo(v); // return which SCC v belongs to
   list  allVOfSCC(id); // it will  takes connected component ID and  returns all the vertices belongs to that CC
   
    boolean addVertex(u);
    boolean addEdge(u, v);
    boolean remEdge(u, v);
 };
 \end{verbatim}
 
\noindent \textbf{\adde:}
At first the $\adde(u, v)$ method starts by checking for the presence of vertices $u$ and $v$ in the vertex list of the SCC graph by invoking the $HelpSearchEdge$ method (Algorithm \ref{helpsearch:Edge}). After this, once again $u$ \& $v$ are validated to be unmarked in the Line \ref{lin:loce8:16}. The reason for this is explained by an example in Figure \ref{fig:noseqhist}. Once the vertices $u$ and $v$ have been validated to be reachable and unmarked in the vertex list, the thread traverses the edge list of vertex $u$ until an edge node with key greater than $v$ has been encountered, say $ecurr$ and it's predecessor say $epred$, locks are obtained on the $epred$ and $ecurr$. The thread does all this without acquiring locks on vertex $u$ and $v$. After this, validation is performed to check if the respective edge nodes are unmarked and reachable. If the validation is successful, the new edge node is added in between $epred$ and $ecurr$ in the edge list of $u$. The \emph{\adde} method is described in the Algorithm

It first If you add an edge between two vertices which belong to some strongly connected component (SCC), then this wont change the number of SCC's in the graph. 

However, the situation gets interesting when you connect two vertices in different SCC's. Once you have found all the SCC's in a graph, you now visualize the graph by collapsing all the vertices into a single node and consider the edges coming from some other SCC's as an inward edges and the ones going out to other SCC's as the outward edges. This will give you a Directed Acyclic Graph (DAG). If you introduce any cycle, of size say n, in this DAG by introducing another edge, this will turn that cycle into one SCC and hence this will result in reducing the number of SCC's by n-1 in the original graph.

\subsection{SCC Algorithms based on Robert Trojan's }

\begin{algorithm}[H]
	\caption{It takes the input graph G = (V, E) and outputs set of strongly connected components (sets of vertices)}
	\label{method:SCCTarjan}
	\begin{algorithmic}[1]
		\Procedure{SCCTarjan($G(V,E$), $n\downarrow, m\downarrow,components\uparrow$ )}{}
	   \State{bool $visited[n]$;}
	   \State{Stack $stack$;}
        \State{int $time\gets 0$;}
        \State{int $lowlink[n]$;}
       % \State{List $components[][]$;}
        \State{int $u\gets0$}
       % \State{List[][]scc(G, n, m)}
        \While{($u<n$)}
        \If{($!visted[u]$)}
        \State{$DFS(u\downarrow$,$components\uparrow)$;}
        \EndIf
        \State{$u\gets u+1$;}
        \EndWhile
        \State{return }
        \EndProcedure
	\end{algorithmic}
\end{algorithm}
%-------------------------------------------------

\begin{algorithm}[H]
	\caption{DFS Method: }
	\label{method:DFS}
	\begin{algorithmic}[1]
	\Procedure{DFS ($u\downarrow$,$components\uparrow)$)}{}
	 \State{$lowlink[u] \gets time++;$}
    \State{$visited[u] \gets true;$}
    \State{$stack.add(u)$;}
    \State{$boolean$ $isComponentRoot \gets true;$;}
    \For{(int v : graph[u])} 
     \If{($!visted[u]$)}
        \State{$DFS(u\downarrow$,$components\uparrow)$;}
    \EndIf
    \If{($lowlink[u] > lowlink[v]$)}
    \State{$lowlink[u] \gets lowlink[v];$}
    \State{$isComponentRoot \gets false;$}
    \EndIf    
    \EndFor
   \If{($isComponentRoot$)}
    \State{component $\gets$ new ArrayLis();}
    \While{($true$)}
    \State{$x \gets stack.pop()$;}
    \State{$component.add(x)$;}
    \State{$lowlink[x] \gets Integer.MAX\_VALUE$;}
     \If{($x = u$)}
     \State{$break$;}
     \EndIf
     \EndWhile
     \State{$components.add(component)$;}
    \EndIf
    \EndProcedure
	\end{algorithmic}
\end{algorithm}
%-------------------------------------------------



\subsection{SCC based on Kosaraju's Algorithm based on coloring}

\begin{enumerate}
    \item Perform a $DFS$ of $G$ and number the vertices in order of finishing time($f_i$).
\item Construct a new directed graph $G^T$ by reversing the direction of every edges in $G$, also called transpose of $G$.
\item Perform a $DFS$ on $G^T$ starting the search from the highest $f_i$ of vertex. If the $DFS$ does not reach all vertices, start the next $DFS$ from the highest numbered remaining vertex.
\item Each tree in the resulting spanning forest is a strong component of $G$.
\end{enumerate}

\begin{algorithm}[H]
	\caption{SCCKosaraju Method Sequential: }
	\label{method:SCCKosaraju}
	\begin{algorithmic}[1]
		\Procedure{SCCKosaraju ($G, n, m, scc[n]$)}{}
		\For{(each node $v$ in $G$)}
		\State{color $v$ gray;}
		\EndFor
		\State $L$ be an empty list;
		\For{(each node $v$ in $G$)}
		\If{(color of $v$ gray)}
		\State {$DFS(G,v)$, appending each node to list $L$ and colored to black.}
		\EndIf
		\EndFor
		\State{construct $G^T$ from $G$}
		\For{(each node $v$ in $G^T$)}
		\State{color $v$ gray;}
		\EndFor
		\State{$index \gets 0$;}
		\For{(each node $v$ in $L$, in reverse order)}
		\If{(color of $v$ gray)}
		\State {$DFS(G^T, v)$, .}
		
		\State{$index \gets index+1;$}
		\EndIf
		\EndFor
	
		\State {return $index$;	} 
		\EndProcedure
	\end{algorithmic}
\end{algorithm}
%-------------------------------------------------
\begin{algorithm}[H]
	\caption{SCC Method Concurrent: Checks whether $u$ and $v$ belongs to same connected components.  }
	\label{method:SCC-concurrent}
	\begin{algorithmic}[1]
		\Procedure{SCC($G, u, v$)}{}
		\State{scan1[] $\gets$ new glist[n]; }
		\State{scan2[] $\gets$ new glist[n; }
		\State{$Contains(u\downarrow, flag1\uparrow)$ ;}
		\State{$Contains(v\downarrow, flag2\uparrow)$ ;}
		\If{(flag1 = false $\vee$ flag2 = false)}
		\State{return false; }
		\EndIf
		\State{$flag3$ $\gets$ Path($u\downarrow$, $v\downarrow$, $scan1\uparrow$);} // path from u to v
		\State{$flag4$ $\gets$ Path($v\downarrow$, $u\downarrow$, $scan2\uparrow$);} // path from v to u
		\If{(flag3 = true $\wedge$ flag4 = true)}
		  \State{return true;} {// u and v belongs to same connected components}
		\Else
		  \State{return false;} 
		\EndIf  
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


\subsection{SCC based on Forward-Backward (FW-BW)\cite{McLendonHPR01}} 

\begin{enumerate}
    \item Select pivot
\item Find all vertices that can be reached from the pivot (descendant ($D$))
\item Find all vertices that can reach the pivot (predecessor ($P$))
\item Intersection of those two sets is an SCC $(S\gets P \cap D)$
\end{enumerate}

There are three distinct sets leftover $(D-S), (P-S)$, and remainder ($R$)

\begin{algorithm}[H]
	\caption{SCCFWBW Method: }
	\label{method:SCCFWBW}
	\begin{algorithmic}[1]
		\Procedure{SCCFWBW ($G, V$)}{}
		\If{(V = 0)}
		\State {return $NULL$;}
		\EndIf
	    \State{Select a Pivot $u\in V$}
	    \State{$D\gets BFS(G(V, E(V)),u)$;}
	    \State{$P\gets BFS(G(V, E'(V)),u)$;}
	    \State{$R\gets (V-(P\cup D))$;}
	    \State{$S \gets (P \cap D$);}
	    \State{SCCFWBW ($G, D-S$)}
	    \State{SCCFWBW ($G, P-S$)}
	    \State{SCCFWBW ($G, R$)}
	    \EndProcedure
	\end{algorithmic}
\end{algorithm}





==> working.tex <==
%\vspace{-2mm}
\section{Working of Concurrent Graph Methods}
\label{sec:working-con-graph-methods}
\vspace{-2mm}
In this section, we describe the implementation of the concurrent graph structure and the working of the various \mth{s}. We represent the graph using adjacency list representation, which is a list of linked lists as illustrated in the Figure \ref{fig:digraph}. The underlying adjacency list implementation is an adaptation of the lazy-list based concurrent set \cite{Heller-PPL2007}. All the fields in the structure are declared atomic. This ensures that operations on these variables happen atomically. In the context of a particular application, the node structure can be easily modified to carry useful data (like weights etc). 

\ignore {
\noindent \textbf{Notations used in PseudoCode:}\\[0.2cm]
$\downarrow$, $\uparrow$ denote input and output arguments to each method respectively. The shared memory is accessed only by invoking explicit \emph{read()} and \emph{write()} methods. The $flag$ is a local variable which returns the status of each operation. We use $e_1$, $e_2$ to represent the $\enode$ reference nodes and $v_1$, $v_2$, $v$ to represent $\vnode$ references. \vspace{-2mm}
%--------------------------------------------------------------------------
%================================================================================
%\begin{flushleft}
%\vspace{-3mm}
\begin{minipage}[t]{6cm}
\null 
 \begin{algorithm}[H]
 \captionsetup{font=scriptsize}
 \caption{\addv  Method: Successfully adds $VNode(key)$ to the vertex list, if it is not present earlier.}
	\label{alg:add:Vertex}
	\begin{algorithmic}[1]
	%\algrestore{locv}
		\scriptsize
		\Procedure{\addv ($key\downarrow$)}{}
		\State {$LocateVertex(key\downarrow,v_1\uparrow,v_2\uparrow )$;} \label{lin:addv2}
		\If {$(read(v_2.val) \neq key$)}  \label{lin:addv3} % \hspace{.5cm} {// not present} 
		\State {$write(v_3, \text{new $\vnode$}(key))$;} \label{lin:addv4} %\hspace{.5cm} {// new vnode created} 
		\State {$write(v_3.vnext, v_2)$;}  \label{lin:addv5} 
		\State {$write(v_1.vnext, v_3)$;}  \label{lin:addv6} %\hspace{.5cm} {// added in the vertex list} 
		\EndIf
		\State {$lock.release(v_1)$;}  \label{lin:addv7}
		\State {$lock.release(v_2)$;}  \label{lin:addv8}
        %\State {$flag \gets true;$}  \label{lin:addv9}
		%\State {$return;$} \label{lin:addv9.1}
        \State {$return$;} 
        \EndProcedure
        \algstore{addv}
	\end{algorithmic}
	\end{algorithm}
\end{minipage}%
\hspace{0.5cm}
%\flushright
\begin{minipage}[t]{6cm}
\null
 \begin{algorithm}[H]
   \captionsetup{font=scriptsize}
   \caption{\remv Method: $\vnode(key)$ gets removed from the vertex list if it is already present. Initially $flag$ is set to $true$.}
	\label{alg:remove:Vertex}
	\begin{algorithmic}[1]
	\algrestore{addv}
	\scriptsize
		\Procedure{\remv ($key\downarrow,flag\uparrow$)}{}
		\State {$ LocateVertex(key\downarrow,v_1\uparrow,v_2\uparrow )$}    \label{lin:remv2}
%			\State{ // $LocateEdge$ return $v_1$ and $v_2$.}
		\If {$(read(v_2.val) = key)$} \label{lin:remf:Vertex}%{ \hspace{.35cm} // present} \label{lin:remv3}
		\State {$write(v_2.marked, true)$;}%{ \hspace{.35cm} // logically removed}
	%	{ /* The key is present and marking the marked field to true, it the linearization point for successful remove vertex. It the logical remove of the vertex from the graph*/}
	\label{lin:remt:Vertex} \label{lin:remv4}
		\State {$write(v_1.vnext, v_2.vnext)$;}  \label{lin:remv5}%\hspace{.5cm} %{// physically removed}
		\State {$lock.release(v_1)$;} \label{lin:remv6}
		\State {$lock.release(v_2)$;} \label{lin:remv7}
		 \State {$RemoveIncomingEdges (key\downarrow)$;}
		%\State{ /* $RemoveIncomingEdges$ removes all incoming edges to $\vnode(key)$.  */}
  %      \State {$flag \gets true;$}  \label{lin:remv8}
%		\State {$return;$} \label{lin:remv8.1}
        \Else 
		\State {$lock.release(v_1)$;} \label{lin:remv10}%
		\State {$lock.release(v_2)$;} \label{lin:remv11}
		\State {$flag \gets false;$}  \label{lin:remv12}%\hspace{.35cm} {// not present}
%		\State {$return;$} \label{lin:remv12.1}   
		\EndIf  
        \State {$return$;}%\hspace{.35cm} {//return flag}
		\EndProcedure
		\algstore{remv}
	\end{algorithmic}
	
  \end{algorithm}
\end{minipage}
%\end{flushleft}
%\hspace{0.5cm}

%==========================================================================================
%-------------------------------------------------------------------------------
%--------------------------------------------------------------------------
%================================================================================
%\begin{flushleft}
%\vspace{-\abovedisplayskip}

\begin{minipage}[t]{6cm}
\null 
 \begin{algorithm}[H]
 \captionsetup{font=scriptsize}
\caption{\adde Method: $\enode(key_2)$ gets added to the edge list of $\vnode(key_1)$, if it is not present. Initially, $flag$ is set to $true$.}
	\label{alg:add:Edge}
	\begin{algorithmic}[1]
	
	%\algrestore{remv}
	\scriptsize
		\Procedure{\adde ($key_1\downarrow$,$key_2\downarrow, flag\uparrow$)}{}
		\State {$LocateEdge(key_1\downarrow, key_2\downarrow, v_1\uparrow, v_2\uparrow, e_1\uparrow, e_2\uparrow, flag\uparrow);$}    \label{lin:adde2}
		%\State{ // $LocateEdge$ return $e_1$ and $e_2$.}
        \If {($flag$ = $false$)} % \hspace{.2cm} {// $\vnode(key_1)$ or $\vnode(key_2)$ not found}
        \State {$return$; }
        \EndIf
        %\State{/* After this line, the method does not return false. It does not matter if the node is there or not.*/}
		\If {$(read(e_2.val) \neq key_2$)} \label{lin:addf:Edge}  \label{lin:adde3}% \hspace{.25cm}  {// $\enode(key_2)$ not present}
		\State {$write(e_3, \text{new $\enode$}(key_2))$;}  \label{lin:adde4}
		\State {$write(e_3.enext, e_2)$;} \label{lin:adde5}
		\State {$write(e_1.enext, e_3)$;} \label{lin:adde6}
		\EndIf  
		\State {$lock.release(e_1)$;} \label{lin:adde7}
		\State {$lock.release(e_2)$;} \label{lin:adde8}
        %\State {$flag \gets true;$}  \label{lin:adde9}
		\State $return$; \label{lin:adde9.1} % \hspace{0.5cm}{// returns flag to be true}
       \EndProcedure
		\algstore{addee}
	\end{algorithmic}
	\end{algorithm}
\end{minipage}%
\hspace{0.5cm}
%\flushright
\begin{minipage}[t]{6cm}
\null
 \begin{algorithm}[H]
   \captionsetup{font=scriptsize}
   \caption{\reme Method: $\enode(key_2)$ gets removed from the edge list of $\vnode(key_1)$, if it is present. Returns successful if the edge is not present earlier.}
	\label{alg:remove:Edge}

	\begin{algorithmic}[1]
	\algrestore{addee}
	\scriptsize
		\Procedure{\reme ($key_1\downarrow$, $key_2\downarrow, flag\uparrow$)}{}
		\State {$LocateEdge(key_1\downarrow, key_2\downarrow, v_1\uparrow, v_2\uparrow, e_1\uparrow, e_2\uparrow, flag\uparrow);$}   \label{lin:reme2}
%		\State{ // $LocateEdge$ return $e_1$ and $e_2$.}
		%\State{/* $\vnode(key_1)$ or $\vnode(key_2)$ not found*/}
       \If {($flag$ = $false$)} 
        \State {$return$;}        
        \EndIf
        \If {$(read(e_2.val) = key_2)$} \label{lin:reme3} %\hspace{.35cm}{ // $\enode(key_2)$ present}
		\State {$write(e_2.marked, true)$;}% \hspace{.35cm} {// logically removed} \label{lin:reme4}
		\State {$write(e_1.enext, e_2.enext)$;} \label{lin:reme5} %\hspace{.5cm} {// physically removed}
       %  \State {$flag \gets true;$}  \label{lin:reme12}
		%\State {return $true$;} \label{lin:reme8}
		\EndIf %\hspace{.35cm}  { // not present}
		\State {$lock.release(e_1)$;} \label{lin:reme10}
		\State {$lock.release(e_2)$;} \label{lin:reme11}
	%	 \State {$flag \gets true;$}  \label{lin:reme12}
		%\State $return$;\label{lin:reme12.1}
		%\EndIf
        \State {$return$;} %\hspace{.35cm} {//  returns flag which is true}
		\EndProcedure
        %\algstore{reme}
	\end{algorithmic}
  \end{algorithm}
\end{minipage}
%\end{flushleft}
%\hspace{0.5cm}
%==========================================================================================
%-------------------------------------------------------------------------------

\begin{algorithm}[H]
	\caption{ValidateVertex Method: Takes two vertices, $v_1, v_2$, each of type $\vnode$ as input and validates for presence in vertex list and returns $true$ or $false$.} 
	\label{validate:Vertex}
	\begin{algorithmic}[1]
	%\algrestore{locv}
	\scriptsize
		\Procedure{ValidateVertex($v_1\downarrow, v_2\downarrow, flag \uparrow$)}{} 
		%\State{// check $v_1$ \& $v_2$ not are marked and $v_1.vnext = v_2$.}
		\If {$(read(v_1.marked) = false) \wedge (read(v_2.marked) = false) \wedge (read(v_1.vnext) = v_2) )$} \label{lin:valv2}
		\State {$flag \gets true;$}  \label{lin:valv3} \hspace{.5cm} {   // validation successful} 
       % \State {$return;$}  \label{lin:valv3.1}
		\Else 
        \State {$flag \gets false;$}  \label{lin:valv5} \hspace{.5cm} {    // validation fails} 
	%	\State {$return$;} \label{lin:valv5.1} 
		\EndIf 
        \State {$return$;} \hspace{.5cm}  {     //return flag}
		\EndProcedure
		\algstore{valv}
	\end{algorithmic}
\end{algorithm}
%--------------------------------------------------------------------------------------------------
\begin{algorithm}[H]
	\caption{LocateVertex Method: Takes $key$ as input and returns the corresponding pair of neighboring $\vnode$ $\langle v_1, v_2 \rangle$. Initially $v_1$ and $v_2$ are set to $null$.}
	\label{locate:Vertex}
	\begin{algorithmic}[1]
	\algrestore{valv}
	\scriptsize
		\Procedure{LocateVertex ($key\downarrow,v_1\uparrow, v_2\uparrow $)}{}
		\While{(true)}
		\State {$v_1 \gets read(\vh)$;} \label{lin:locv3}
		\State {$v_2 \gets read(v_1.vnext)$;} \label{lin:locv4}
		\While{$(read(v_2.val) < key)$} \label{lin:locv5} \hspace{.4cm} {         // search without acquiring lock}
		\State {$v_1 \gets v_2$;} \label{lin:locv6}
		\State {$v_2 \gets read(v_2.vnext)$;} \label{lin:locv7} 
		\EndWhile
		\State {$lock.acquire(v_1)$;} \label{lin:locv9}
		\State {$lock.acquire(v_2)$;} \label{lin:locv10}
		\State{/* If ValidateVertex returns true, then it returns. */}
		%\State {/*If flag is true, return*/}
		\If{($ValidateVertex(v_1 \downarrow, v_2$ $\downarrow$, $flag \uparrow$))} \hspace{.1cm} 
		%\Comment{flag set by ValidateVertex} 
		\label{lin:locv11} 
		%\State return; \label{lin:locv12}  {//it returns with $(v_1,v_2)$ if validation succeeds.}
		\State{$ return;$}
		\Else   
		\State {$lock.release(v_1)$;} \label{lin:locv14}
		\State {$lock.release(v_2)$;} \label{lin:locv15} \hspace{.5cm} {//validation failed, try again}
		\EndIf
		\EndWhile
		\EndProcedure
		\algstore{locv}
	\end{algorithmic}
\end{algorithm}
}


\ignore{
\begin{algorithm}
	\caption{\addv  Method: Successfully adds $VNode(key)$ to the vertex list, if it is not present earlier.}
	\label{alg:add:Vertex}
	\begin{algorithmic}[1]
	\algrestore{locv}
		\scriptsize
		\Procedure{\addv ($key\downarrow$)}{}
		\State {$LocateVertex(key\downarrow,v_1\uparrow,v_2\uparrow )$;} 
		\label{lin:addv2}
		\If {$(read(v_2.val) \neq key$)}  \label{lin:addv3}  \hspace{.5cm} {// not present} 
		\State {$write(v_3, \text{new $\vnode$}(key))$;} \label{lin:addv4} \hspace{.5cm} {// new vnode created} 
		\State {$write(v_3.vnext, v_2)$;}  \label{lin:addv5} 
		\State {$write(v_1.vnext, v_3)$;}  \label{lin:addv6} \hspace{.5cm} {// added in the vertex list} 
		\EndIf
		\State {$lock.release(v_1)$;}  \label{lin:addv7}
		\State {$lock.release(v_2)$;}  \label{lin:addv8}
        %\State {$flag \gets true;$}  \label{lin:addv9}
		%\State {$return;$} \label{lin:addv9.1}
        \State {$return$;} 
        \EndProcedure
        \algstore{addv}
	\end{algorithmic}
\end{algorithm}
}
\subsection{\emph{Update Vertex Methods} - \addv \& \remv}
\label{sec:working-con-graph-methods:add}
%\textbf{Working of the Add() methods:}\\[0.1cm]
\noindent The $\addv(u)$ method is similar to the add method of concurrent set implemented using lazy linked list\cite{Heller-PPL2007}. When a thread wants to add a vertex to the concurrent graph, it traverses the vertex list without acquiring any locks until it finds a vertex with its key greater than or equal to $u$, say $ucurr$ and it's predecessor, say $upred$. It acquires locks on the vertices $upred$ and $ucurr$ itself. It validates to check if $ucurr$ is reachable from $upred$, and if both the vnodes have not been deleted (marked). The algorithm maintains an invariant that all the unmarked vertex nodes are reachable. 
\noindent If the validation succeeds, the thread adds the vertex $u$ between $upred$ and $ucurr$ in the vertex list and returns true after unlocking the vertices. If it fails, the thread starts the traversal over after unlocking the locked vertices. The \emph{\addv} method is described\footnote{Due to lack of space, all the pseudo code and examples are given in the Appendix Section, at the end of the paper.} in the Algorithm \ref{alg:add:Vertex}. \\
\ignore{
%---------------------------------------------------
\begin{algorithm}[H]
	\caption{RemoveIncomingEdge Method: This method helps remove all the incoming edges of a deleted vertex $vnode(key)$ from the graph.}
	\label{alg:HelpRemoveIncomingEdgex}
	\scriptsize
	\begin{algorithmic}[1]
	\algrestore{addv}
		\Procedure{RemoveIncomingEdge ($key\downarrow$)}{}
		\State $temp \gets read(\vh)$;\hspace{.5cm} {// Starting from $\vh$}
        \While {($read(temp.vnext) \neq NULL$)}  
   		\While{($true$)}
   		\State {$e_1 \gets read(temp.\eh)$;} \label{lin:loce17.1}
        \State {$e_2 \gets read(e_1.enext)$;}\label{lin:loce18.1}
		\While{$(read(e_2.val) < key)$}\label{lin:loce19.1}
		\State {$e_1 \gets e_2$;} \label{lin:loce20.1}
		\State {$e_2 \gets read(e_2.enext)$;} \label{lin:loce21.1}
		\EndWhile
        \State {$lock.acquire(e_1)$;}\label{lin:loce23.1}
		\State {$lock.acquire(e_2)$;}\label{lin:loce24.1}
		\If{($ValidateEdge(e_1, e_2$))}\label{lin:loce25.1} 
		\If {$(read(e_2.val) = key)$} \label{lin:reme3.1} \hspace{.5cm} {// key is present} 
		\State {$write(e_2.marked, true)$;} \label{lin:reme4.1}\hspace{.5cm} {// logically removed} 
		\State {$write(e_1.enext, e_2.enext)$;}\hspace{.5cm} {// physically removed}  \label{lin:reme5.1}
       %  \State {$flag \gets true;$}  \label{lin:reme12}
		%\State {return $true$;} \label{lin:reme8}
		\EndIf
		\EndIf
		\State {$lock.release(e_1)$;} \label{lin:reme6.1}
		\State {$lock.release(e_2)$;} \label{lin:reme7.1}
		\EndWhile
        \State $temp \gets temp.vnext$ 
        \EndWhile
       % \State {$flag \gets true;$}  \label{lin:remv8}
		\State {$return$;} 
		\EndProcedure
		\algstore{remie}
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}[H]
	\caption{\remv Method: $\vnode(key)$ gets removed from the vertex list if it is already present. Initially $flag$ is set to $true$.}
	\label{alg:remove:Vertex}
	\begin{algorithmic}[1]
	\algrestore{remie}
	\scriptsize
		\Procedure{\remv ($key\downarrow,flag\uparrow$)}{}
		\State {$ LocateVertex(key\downarrow,v_1\uparrow,v_2\uparrow )$}    \label{lin:remv2}
%			\State{ // $LocateEdge$ return $v_1$ and $v_2$.}
		\If {$(read(v_2.val) = key)$} \label{lin:remf:Vertex}{ \hspace{.35cm} // present} \label{lin:remv3}
		\State {$write(v_2.marked, true)$;}{ \hspace{.35cm} // logically removed}
	%	{ /* The key is present and marking the marked field to true, it the linearization point for successful remove vertex. It the logical remove of the vertex from the graph*/}
	\label{lin:remt:Vertex} \label{lin:remv4}
		\State {$write(v_1.vnext, v_2.vnext)$;}  \label{lin:remv5}\hspace{.5cm} {// physically removed}
		\State {$lock.release(v_1)$;} \label{lin:remv6}
		\State {$lock.release(v_2)$;} \label{lin:remv7}
		 \State {$RemoveIncomingEdges (key\downarrow)$;}
		\State{ /* $RemoveIncomingEdges$ removes all incoming edges to $\vnode(key)$.  */}
  %      \State {$flag \gets true;$}  \label{lin:remv8}
%		\State {$return;$} \label{lin:remv8.1}
        \Else 
		\State {$lock.release(v_1)$;} \label{lin:remv10}%
		\State {$lock.release(v_2)$;} \label{lin:remv11}
		\State {$flag \gets false;$}  \label{lin:remv12}\hspace{.35cm} {// not present}
%		\State {$return;$} \label{lin:remv12.1}   
		\EndIf  
        \State {$return$;}\hspace{.35cm} {//return flag}
		\EndProcedure
		\algstore{remv}
	\end{algorithmic}
\end{algorithm}
}
From the structure of \emph{\vnode} class, we know that each $\vnode$ has a boolean \emph{marked} field in Table \ref{tab:struct:vertex-edge}. The removal of a $\vnode$, say $u$ happens in two steps like in the lazy linked list \cite{Heller-PPL2007}: (1) The $\vnode$ $u$'s marked field is first set to true and it referred to as logical removal. This ensures that if any edge is being added or removed concurrently corresponding to that vertex will fail in the validation process after checking the marked field at the Line \ref{lin:valv2} in the Algorithm \ref{validate:Vertex}. (2) Then, the pointers are changed so that $u$ is removed from the \vlist(Line \ref{lin:remv4}). This is referred to as physical deletion, then it changes the pointer(Line \ref{lin:remv5}) of the predecessor of the marked node to its successor so that the deleted node is no longer reachable in the \vlist. To achieve this, $\remv(u)$ method proceeds similar to the $\addv(u)$. The thread iterates through \vlist until it identifies the vertex $u$ to be deleted. Then after $u$ and its predecessor are locked, then logical removal occurs by setting the marked field to $true$. The \emph{\remv} method is described in the Algorithm \ref{alg:remove:Vertex}. \\ 
%-------------------------------------------------
 After the physical deletion of the vertex $u$, the vertices should be removed from the edge-list of all the other nodes $v$ from which the incoming edges to $u$. This is described by the $RemoveIncomingEdge$ method (Algorithm \ref{alg:HelpRemoveIncomingEdgex}). This is done by performing a traversal of the entire \vlist, to check if the deleted vertex contains an edge node in their edge list. If such an edge node is present, locks are obtained on the \emph{enodes} $e_1$ and $e_2$ in the Line \ref{lin:loce23.1} and \ref{lin:loce24.1} respectively of the vertex $v$ and then this edge node $e_2$ is deleted by setting the marked to $true$ (logical removal) and then physically deleted. The physical deletion does not remove the $\vnode$ from the memory as we are not doing any garbage collection. All deleted \emph{vnodes} are not reachable from the \emph{$\vh$} but they are present in the system.
%The implementation is available at \cite{Pdcrl-ConcurrentGraphDS2017}. 
 
\subsection{\emph{Update Edge Methods} - \adde \& \reme }
\label{sec:working-con-graph-methods:remove}

\ignore{
\begin{algorithm}[H]
\scriptsize
	\caption{ValidateEdge Method: Takes two $ENode$ $e_1, e_2$ and validates for presence in edge list.}
	\label{validate:Edge}
	\begin{algorithmic}[1]
	\algrestore{remv}
		\scriptsize
		\Procedure{$ValidateEdge(e_1\downarrow, e_2\downarrow, flag\uparrow$)}{}
	%	\State{// check $e_1$ \& $e_2$ are not marked and $e_1.enext = e_2$.}
		\If {$(read(e_1.marked) = false) \wedge (read(e_2.marked) = false) \wedge (read(e_1.enext) = e_2$))} \label{lin:vale2}
        \State {$flag \gets true;$}  \label{lin:vale3}\hspace{.5cm}{// validation successful} 
		%\State $return;$  \label{lin:vale3.1}
		\Else 
        \State {$flag \gets false;$}  \label{lin:vale5}\hspace{.5cm} {//validation fails} 
		%\State $return$;\label{lin:vale5.1}
		\EndIf
        \State {$return$;} \hspace{.5cm} {//return flag}
		\EndProcedure
		\algstore{vale}
	\end{algorithmic}
\end{algorithm}

%--------------------------------------------------------------------------------------------------

%--------------------------------------------------------
\begin{algorithm}[H]
	\caption{HelpSearchEdge Method: This method helps to optimise searching of edge vertices. It compare the $key_1$ and $key_2$, starts searching based on  smaller key value.  Takes two keys, $key_1$ and $key_2$, as input and returns the $\vnode$ $\langle v_1, v_2 \rangle$ corresponding to them. Initially $v_1, v_2$ are set to $null$ and $flag$ is set to $true$.}
	\label{helpsearch:Edge}
	\begin{algorithmic}[1]
	\algrestore{vale}
		\scriptsize
		\Procedure{HelpSearchEdge ($key_1 \downarrow, key_2\downarrow, v_1\uparrow, v_2\uparrow, flag \uparrow$)}{}
		
        \If{$(key_1 < key_2)$}
        \State {$v_1 \gets read(\vh)$;}\hspace{.5cm} {// starting from $\vh$ } %\label{lin:loce3} 
        \While{$(read(v_1.val) < key_1)$} %\label{lin:loce4}
		\State {$v_1 \gets read(v_1.vnext)$;} %\label{lin:loce5}
		\EndWhile
        \If{($read(v_1.val$ $\neq$ $key_1$) $\vee$ ($read(v_1.marked$))} \label{lin:helploce8}\hspace{.5cm} {//$\vnode(key_1)$ not present or marked }
        \State {$flag \gets false$;} %\label{lin:loce8}
        \State {$return$;}
        \EndIf
        \State {$v_2 \gets read(v_1.vnext)$;}%\label{lin:loce10}
		\While{$(read(v_2.val) < key_2)$} %\label{lin:loce11}
		\State {$v_2 \gets read(v_2.vnext)$;} %\label{lin:loce12}
		\EndWhile
        \If{($read(v_2.val$ $\neq$ $key_2$) $\vee$ ($read(v_2.marked$))}\label{lin:helploce16}\hspace{.5cm} {// $\vnode(key_2)$ not present or marked }
        \State {$flag \gets false$;} %\label{lin:loce15}
        \State {$return$;}
        \EndIf
        %\State {$return$;}
        \Else 
        \State {$v_2 \gets read(\vh)$;}\hspace{.5cm} {// starting from $\vh$ }%\label{lin:loce10.1}
		\While{$(read(v_2.val) < key_2)$} %\label{lin:loce11.1}
		\State {$v_2 \gets read(v_2.vnext)$;} %\label{lin:loce12.1}
		\EndWhile
        \If{($read(v_2.val$ $\neq$ $key_2$) $\vee$ ($read(v_2.marked$))} \label{lin:helploce16.1}\hspace{.5cm} {//$\vnode(key_2)$ not present or marked }
        \State {$flag \gets false$;} %\label{lin:loce15.1}
       \State {$return$;}
        \EndIf
        \State {$v_1 \gets read(n_v.vnext)$;}%\label{lin:loce3.1}
        \While{$(read(v_1.val) < key_1)$} %\label{lin:loce4.1}
		\State {$v_1 \gets read(v_1.vnext)$;} %\label{lin:loce5.1}
		\EndWhile
        \If{($read(v_1.val$ $\neq$ $key_1$) $\vee$ ($read(v_1.marked$))}  \label{lin:helploce8.1}\hspace{.5cm} {//$\vnode(key_1)$ not present or marked }
        \State {$flag \gets false$;} %\label{lin:loce8.1}
        \State {$return$;}
       % \State {$return$;}
        \EndIf
        \EndIf
      	\EndProcedure
      	\algstore{hse}
	\end{algorithmic}
\end{algorithm}
%\vspace{-1mm}
}
\noindent The $\adde(u, v)$ method starts by checking for the presence of vertices $u$ and $v$ in the vertex list of the graph by invoking the $HelpSearchEdge$ method (Algorithm \ref{helpsearch:Edge}). Once the vertices $u$ and $v$ are validated to be reachable and unmarked in the vertex list, the thread traverses the edge list of vertex $u$ to add an edge node for the vertex $v$. The thread does all this without acquiring locks on $u$ and $v$. Before doing this it is necessary to check the vnodes are marked or not, as while adding edge $v$ in the $u$ list, some other thread could have deleted the vertices $u$ or/and $v$. So by checking $(read(v_1.marked)$ $\vee$ $read(v_2.marked))$ in the Line \ref{lin:loce8:16}, we ensure that the vertices were not deleted before beginning of the \emph{\adde} method. Then after the searching of the vnode $v$ continues until an edge node with key greater than $v$ has been encountered, say $ecurr$ and it's predecessor say $epred$, locks are obtained on the $epred$ and $ecurr$. After this, validation is performed to check if the respective edge nodes are unmarked and reachable. If the validation is successful, the new edge node is added in between $epred$ and $ecurr$ in the edge list of $u$. The \emph{\adde} method is described in the Algorithm \ref{alg:add:Edge}.

\ignore{
\begin{figure}[th]
	\centerline{\scalebox{0.5}{\input{figs/false.pdf_t}}}
	\caption{An example with no possible sequential history. Thread $T_1$ calls the \adde(u, v, true) method, for this at first it invoked LocateEdge and then invokes HelpLocateEdge. Before executing Line \ref{lin:helploce16} thread $T_2$ calls \remv(u, true) and it successful removed the vertex $u$. Also before iexecuting Line \ref{lin:helploce16} by $T_1$, thread $T_3$ can invoked \addv(v, true) and it successfully added the vertex $v$. So, now the $T_1$ successfully tested for the presence of vertices $u$ and $v$, and then it tries to add edge $(u,v)$, which is incorrect as it violates the sequential history.}
	\label{fig:noseqhist}
\end{figure}
}
\ignore{
%--------------------------------------------------------
\begin{algorithm}[H]
	\caption{LocateEdge Method: Takes two keys, $key_1$ and $key_2$, as input and returns the pair of adjacent $\enode$ $\langle e_1, e_2 \rangle$. If $\vnode$ $v_1$ or $v_2$ or $\enode$ $e_2$ is not present, it returns false. Initially enodes $e_1, e_2$ are set to $null$ and $flag$ is set to $true$.}
	\label{locate:Edge}
	\begin{algorithmic}[1]
		\scriptsize
		\algrestore{hse}
		\Procedure{LocateEdge ($key_1 \downarrow, key_2\downarrow, v_1\uparrow, v_2\uparrow, e_1\uparrow, e_2\uparrow, flag\uparrow$)}{}
        \State{$ HelpSearchEdge (key_1 \downarrow, key_2\downarrow, v_1\uparrow, v_2\uparrow, flag \uparrow$);}
        \If {($flag$ = $false$)}
        \State {$return$; }\hspace{.4cm} { // $v_1$ or $v_2$ not found, returns flag}
        \EndIf
        \State{/*This lines ensures both the vertices $v_1$ \& $v_2$ have been added to the system by this time  and are not marked*/}
        \If {$(read(v_1.marked)$ $\vee$ $read(v_2.marked))$}  \label{lin:loce8:16}
        \State {$flag \gets false$;} 
        \State {$return$; }
        \EndIf

		\State{/* Helping for search edge, is a supporting method for locate edge. It locates the vertices $v_1$ \& $v_2$*/}
        \While{(true)}
		
		\State {$e_1 \gets read(v_1.enext)$;} \label{lin:loce17}
        \State {$e_2 \gets read(e_1.enext)$;}\label{lin:loce18}
        \State{ /* Search $\enode(key_2)$ without acquiring any locks*/}
		\While{$(read(e_2.val) < key_2)$}\label{lin:loce19}
		\State {$e_1 \gets e_2$;} \label{lin:loce20}
		\State {$e_2 \gets read(e_2.enext)$;} \label{lin:loce21}
		\EndWhile
        \State {$lock.acquire(e_1)$;}\label{lin:loce23}
		\State {$lock.acquire(e_2)$;}\label{lin:loce24}
		\If{($ValidateEdge(e_1 \downarrow, e_2 \downarrow, flag \uparrow$))}\label{lin:loce25}
        %\State{$flag \gets true$}; 
		\State return;\label{lin:loce26} \hspace{.4cm} {// returns true if validation succeeds.}
		\Else 
		\State {$lock.release(e_1)$;}\label{lin:loce28}
		\State {$lock.release(e_2)$;}\label{lin:loce29} \hspace{.4cm} {// validation failed, try again}
		\EndIf
		\EndWhile
		\EndProcedure
		\algstore{loce}
	\end{algorithmic}
\end{algorithm}
%\vspace{-2mm}

%-------------------------------------------------
\begin{algorithm}[H]
	\caption{\adde Method: $\enode(key_2)$ gets added to the edge list of $\vnode(key_1)$, if it is not present. Initially, $flag$ is set to $true$.}
	\label{alg:add:Edge}
	\begin{algorithmic}[1]
	
	\algrestore{loce}
	\scriptsize
		\Procedure{\adde ($key_1\downarrow$,$key_2\downarrow, flag\uparrow$)}{}
		\State {$LocateEdge(key_1\downarrow, key_2\downarrow, v_1\uparrow, v_2\uparrow, e_1\uparrow, e_2\uparrow, flag\uparrow);$}    \label{lin:adde2}
		%\State{ // $LocateEdge$ return $e_1$ and $e_2$.}
        \If {($flag$ = $false$)} \hspace{.2cm} {// $\vnode(key_1)$ or $\vnode(key_2)$ not found}
        \State {$return$; }
        \EndIf
        \State{/* After this line, the method does not return false. It does not matter if the node is there or not.*/}
		\If {$(read(e_2.val) \neq key_2$)} \label{lin:addf:Edge}  \label{lin:adde3} \hspace{.25cm}  {// $\enode(key_2)$ not present}
		\State {$write(e_3, \text{new $\enode$}(key_2))$;}  \label{lin:adde4}
		\State {$write(e_3.enext, e_2)$;} \label{lin:adde5}
		\State {$write(e_1.enext, e_3)$;} \label{lin:adde6}
		\EndIf  
		\State {$lock.release(e_1)$;} \label{lin:adde7}
		\State {$lock.release(e_2)$;} \label{lin:adde8}
        %\State {$flag \gets true;$}  \label{lin:adde9}
		\State $return$; \label{lin:adde9.1} \hspace{0.5cm}{// returns flag to be true}
       \EndProcedure
		\algstore{adde}
	\end{algorithmic}
\end{algorithm}
}
%\vspace{-1mm}

\noindent In $\reme(u,v)$, the $\enode$ $v$ is removed from $u$'s \elist. This method works similar to $\remv$ \mth. It proceeds in two phases: first logical removal of the \enode $v$ by setting the mark field. Then, $v$ is removed physically from $u$'s \elist by changing the pointers. Unlike $\remv$, the physical removal is simpler as there is no other extra work to be done. This is because the edges in the concurrent graph are directed and only one edge needs to be removed from one list.

\noindent To achieve this, the $\reme(u,v)$ method proceeds similar to the $\adde(u,v)$ by traversing the vertex list in the graph, without acquiring any locks and then verifying that the vertices $u$ and $v$ are indeed present in the graph. The thread then traverses the edge list of $u$ (without acquiring locks) to identify the $epred$ \& $ecurr$ edge nodes. Once these nodes have been locked and validated (for reachability), logical removal occurs and then physical deletion of edge nodes place immediately after logical removal. The \emph{\reme} method is described in the Algorithm \ref{alg:remove:Edge}. %Physical deletion involves changing the pointer of the predecessor of the marked node to its successor so that the deleted node is no longer reachable in the edge list. 

%\vspace{-2mm}
\ignore{
%-------------------------------------------------
\begin{algorithm}[H]
	\caption{\reme Method: $\enode(key_2)$ gets removed from the edge list of $\vnode(key_1)$, if it is present. Returns successful if the edge is not present earlier.}
	\label{alg:remove:Edge}

	\begin{algorithmic}[1]
	\algrestore{adde}
	\scriptsize
		\Procedure{\reme ($key_1\downarrow$, $key_2\downarrow, flag\uparrow$)}{}
		\State {$LocateEdge(key_1\downarrow, key_2\downarrow, v_1\uparrow, v_2\uparrow, e_1\uparrow, e_2\uparrow, flag\uparrow);$}   \label{lin:reme2}
%		\State{ // $LocateEdge$ return $e_1$ and $e_2$.}
		\State{/* $\vnode(key_1)$ or $\vnode(key_2)$ not found*/}
       \If {($flag$ = $false$)} 
        \State {$return$;}        
        \EndIf
        \If {$(read(e_2.val) = key_2)$} \label{lin:reme3} \hspace{.35cm}{ // $\enode(key_2)$ present}
		\State {$write(e_2.marked, true)$;} \hspace{.35cm} {// logically removed} \label{lin:reme4}
		\State {$write(e_1.enext, e_2.enext)$;} \label{lin:reme5}\hspace{.5cm} {// physically removed}
       %  \State {$flag \gets true;$}  \label{lin:reme12}
		%\State {return $true$;} \label{lin:reme8}
		\EndIf \hspace{.35cm}  { // not present}
		\State {$lock.release(e_1)$;} \label{lin:reme10}
		\State {$lock.release(e_2)$;} \label{lin:reme11}
	%	 \State {$flag \gets true;$}  \label{lin:reme12}
		%\State $return$;\label{lin:reme12.1}
		%\EndIf
        \State {$return$;} \hspace{.35cm} {//  returns flag which is true}
		\EndProcedure
        \algstore{reme}
	\end{algorithmic}
	
\end{algorithm}
%\vspace{-3mm}
}
\vspace{-2mm}
\subsection{\emph{Read-Only Methods} - \conv \& \cone}
\noindent Methods $\conv(u)$ and $\cone(u,v)$, as described in Algorithm \ref{contains:Vertex} and \ref{contains:Edge} respectively, traverse the graph without acquiring any locks. These methods return $true$ if the vertex/edge node it was searching for is present and unmarked in the graph and otherwise returns $false$. 


\ignore{
The $\conv(u)$ method works similar to the wait-free contains of lazy linked list. It proceeds by scanning the \vlist, without acquiring any locks until it encounters a \vnode of key greater than or equal to $u$. It returns $true$ if the \vnode it was searching for is present and unmarked in the graph and otherwise $false$. The \conv method is described in the Algorithm \ref{contains:Vertex}.\\
Similarly, the $\cone(u, v)$ method first scans the \vlist like \conv for each vertex $u$ and $v$ and checks both the vertices are present and unmarked. This work has been done by the $HelpSearchEdge$ method described in the Algorithm \ref{helpsearch:Edge}. This method helps to optimise searching of edge vertices. It compares the key value of $u$ and $v$ and starts searching based on smaller key value. Based on the status of $flag$ in the Line \ref{lin:reme2} it decides whether it will scan the \elist of \vnode $u$. If $flag$ is $false$ it directly returns in the Line \ref{lin:reme2.1}, else it starts scanning in the \elist of \vnode $u$ from the Line \ref{lin:cone17}-\ref{lin:cone17.1}. While scanning it ignores the \enodes which are marked or not and continue until it finds a \enode with a key value greater than or equal. It traverse the \elist without acquiring any locks on \enode. It returns $true$ if the \enode it was searching for is present and unmarked in the \elist of \vnode $u$ and otherwise returns $false$. The \cone method is described in the Algorithm \ref{contains:Edge}.

}
%\noindent Methods $\conv(u)$ and $\cone(u,v)$, as described in Algorithm \ref{contains:Vertex} and \ref{contains:Edge} respectively, traverse the graph without acquiring any locks. These methods return $true$ if the vertex/edge node it was searching for is present and unmarked in the graph and otherwise returns $false$.

\ignore{
%-------------------------------------------------
\begin{algorithm}[H]
	\caption{\conv Method: Returns $true$ if $\vnode(key)$ is present in vertex list and returns $false$ otherwise.}
	\label{contains:Vertex}
	\begin{algorithmic}[1]
	\algrestore{reme}
	\scriptsize
		\Procedure{\conv ($key\downarrow, flag\uparrow$)}{}
		\State {$v \gets read(\vh);$}   \label{lin:conv2}
		\While {$(read(v.val) < key)$} \label{lin:conv3}
		\State {$v \gets read(v.vnext);$} \label{lin:conv4}
		\EndWhile  \label{lin:conv5}
		\If{ $((read(v.val) \neq key$) $\vee$ ($read(v.marked)))$}\label{lin:conv6} 
         \State {$flag \gets false;$}  \label{lin:conv7}
		%\State {$return;$} \label{lin:conv7.1}
		\Else
		 \State {$flag \gets true;$}  \label{lin:conv9}
		%\State {$return;$} \label{lin:conv9.1}
		\EndIf
        \State {$return$;} 
		\EndProcedure
		\algstore{conv}
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
	\caption{\cone Method: Returns $true$ if $\enode(key_2)$ is part of the edge list of $\vnode(key_1)$ and returns $false$ otherwise.}
	\label{contains:Edge}
	\begin{algorithmic}[1]
	\algrestore{conv}
	\scriptsize
		\Procedure{\cone ($key_1\downarrow, key_2\downarrow, flag\uparrow$)}{}
        \State{$ HelpSearchEdge (key_1 \downarrow, key_2\downarrow, v_1\uparrow, v_2\uparrow, flag \uparrow$);}
        \State{/* $\vnode(key_1)$ or $\vnode(key_2)$ not found */}
        \If {$(flag$ = false)} 
        \State{$return$;}
        \EndIf
        \State {$e \gets read(v_1.enext)$;}\label{lin:cone16}
       	\While{$(read(e.val) < key_2)$} \label{lin:cone17}
		\State {$e \gets read(e.enext)$;} \label{lin:cone18}
		\EndWhile \label{lin:cone17.1}
	  	\If{ $((read(e.val) \neq key$) $\vee$ ($read(e.marked)))$}      \label{lin:cont-tf:Edge} \label{lin:cone151}
 
	%	\If {$(read(e.val) \neq key) \vee (read(e.marked))$} 
		 \State {$flag \gets false;$}\label{lin:cone21}
     %   \State $return;$ \label{lin:cone21.1}
		\Else
		 \State {$flag \gets true;$}\label{lin:cone23}
    %    \State $return;$ \label{lin:cone23.1}
		\EndIf
       \State {$return$;} 
		\EndProcedure
		\algstore{cone}
	\end{algorithmic}
\end{algorithm}
}
%It can be seen that all the update calls are blocking (use locks) and they are deadlock-free. All the methods described above are linearizable. The proof sketch is described in the technical report\cite{PeriSS16}.
\vspace{-2mm}
\subsection{Correctness: Linearization Points}
\noindent
In this subsection, we define the \textit{Linearization Points(LP)} of all methods of our concurrent graph data structure. 
\noindent The linearization point of $\addv(u)$ method is $write(v_1.vnext, v_3)$ event in Line \ref{lin:addv6}. Line \ref{lin:addv6} implies that the key $u$ is not already present and the effect of this method actually happens at this line, such that a new vertex node is now made reachable from $\vh$ of the vertex list. It can be seen that $\addv (u)$ never returns false which follows from the \sspec.

\noindent For a successful $\remv(u)$ call, the linearization point occurs when the deletion of the key $u$ succeeds i.e. $write(v_2 .marked, true)$ in Line \ref{lin:remv4}, this means the key $u$ is already present in the vertex list. An unsuccessful call is linearized at $read(v_2.val)$ in Line \ref{lin:remv3} where the key $u$ is found to be not present in the vertex list. 

\noindent The successful return of $\conv(u)$ method is linearized when the key $u$ is found to be unmarked in the vertex list i.e. at $read(u.marked)$ in Line \ref{lin:conv6}. We linearize an unsuccessful $\conv$ method call within its execution interval at the earlier of the following points; (1) if no successful concurrent add vertex (lying between the first read of a shared variable in the method until $LP$) on $u$, the $LP$ is defined to be later of $read(n.val)$ not equal to $u$ or $read(n.marked)$ equal to $true$ in Line \ref{lin:conv6}, depending upon the execution. (2) if there is a successful concurrent add vertex on $u$, the $\conv(u)$ is linearized at the point immediately before the $LP$ of the successful concurrent add vertex $u$. This $LP$ is similar to $LP$ of contains in lazy list implementation of the concurrent set \cite{Heller-PPL2007}. Figure \ref{fig:lpcase8} illustrates why a concurrent $\addv$ must be considered while linearizing an unsuccessful $\conv$ \mth.
\ignore{
\begin{figure}[H]
\captionsetup{font=scriptsize}
 \centerline{\scalebox{0.5}{\input{figs/LPCase8.pdf_t}}}
  \caption{An execution of two concurrent operations  $T_1.\conv(7, false)$ and $T_2.\addv(7, true)$. Figure (a) shows that $T_1$ is traversing the vertex list, but these vertices have been deleted consecutively. Meanwhile, some more vertices are added to the vertex list. Now, $T_2$ starts searching for the location to add vertex $7$ in the vertex list. Figure (b) depicts that $T_2$ has successfully added the vertex in the vertex list. Unfortunately, $T_1$ locates a vertex greater than the key value it was looking for, so it returns $false$. The sequential history: $T_2.\addv(7, true)$ $<_H$ $T_1.\conv(7, false)$ (ordered by their execution) is not linearizable. Figure (c) depicts the correct $LP$ order.}
  \label{fig:lpcase8}
\end{figure}
}
\noindent We linearize a successful $\adde(u,v)$ method call within its execution interval at the earlier of the following points; (1) if there is no successful concurrent delete vertex on $u$ and $v$, the $LP$ is defined as the last of $read(e_2.val)$ in Line \ref{lin:adde3} and $write(e_1.enext, e_3)$ in Line \ref{lin:adde6},  depending upon the execution. If the last line to execute is Line \ref{lin:adde3}, the edge $(u,v)$ is present in the edge list of the vertex $u$. Whereas, Line \ref{lin:adde6} implies that the edge $(u,v)$ was not present earlier and this line adds a new edge node $(u,v)$ such that it is now reachable from $\vh$ of the vertex list. (2) if there is a successful concurrent delete vertex on $u$ or $v$ or both, the $LP$ is the point immediately before the first $LP$ of successful concurrent delete on vertex $u$ or $v$.
\noindent Figure \ref{fig:lpcase1} illustrates why a concurrent $\remv$ must be considered while linearizing a successful $\adde$ \mth. Suppose the point where the edge $(5, 7)$ is added to the graph is considered as a LP while there is a concurrent $\remv(7)$. The example shown shows that this \lp will be wrong, since the $\adde$ returns $true$ after successful deletion of the corresponding vertex. 

\ignore{
\begin{figure}[H]
\captionsetup{font=scriptsize}
 \centerline{\scalebox{0.5}{\input{figs/LPCase1.pdf_t}}}
  \caption{An execution of two concurrent operations  $T_1.\remv(7, true)$ and $T_2.\adde(5,7, true)$. Figure (a) shows that $T_2$ has validated vertices $5$ and $7$ for presence in the vertex list and proceeds to add an edge $(5, 7)$. Meanwhile, when $T_1$ is traversing the edge list of vertex $5$ and has marked the vertex $7$. Figure (b) depicts that $LP$ of $\remv(7, true)$ (logical removal) happens before the (wrong) $LP$ of $\adde(5,7, true)$. The sequential history: $T_1.\remv(7, true)$ $<_H$ $T_2.\adde(5,7,true)$  (ordered by their execution) is not linearizable. Figure (c) depicts the correct $LP$ order.}
  \label{fig:lpcase1}
\end{figure}
}
\noindent For an unsuccessful $\adde(u,v)$ call, the $LP$ is defined to be within its execution interval at the earlier of the following points; (1) if there is no successful concurrent add vertex on $u$ and $v$, $LP$ is the, (a) last of $read(u.val)$ in Line \ref{lin:helploce8}/\ref{lin:helploce8.1} where $u$ is not found in vertex list, (b) $read(u.marked)$ in Line \ref{lin:helploce8}/\ref{lin:helploce8.1} where $u$ is found to be marked, (c) $read(v.val)$ in Line \ref{lin:helploce16}/\ref{lin:helploce16.1} where $v$ is not found in the vertex list, (d) $read(v_2.marked)$ in Line \ref{lin:helploce16}/ \ref{lin:helploce16.1} where $v$ is found to be marked, (e) $read(v_1.marked)$ in Line  \ref{lin:loce8:16} or $read(v_1.marked)$ in Line \ref{lin:loce8:16}, depending upon the execution. (2) if there is a successful concurrent add vertex on $u$ or $v$ or both, it is linearized at the point immediately before the $LP$ of the first successful concurrent add vertex on $u$ or $v$. Figure \ref{fig:lpcase3} illustrates how to linearize an unsuccessful $\adde$ \mth in presence of a concurrent $\addv$. Also it  shows the case of concurrent $\reme$ as well since its $\lp$ is very similar to $\adde$. 
\ignore{
\begin{figure}[H]
\captionsetup{font=scriptsize}
 \centerline{\scalebox{0.5}{\input{figs/LPCase3.pdf_t}}}
  \caption{
  An execution of three concurrent operations  $T_1:\addv(7, true)$, $T_2:\adde(5, 7, false)$ and $T_3:\reme(5, 7, false)$. Figure (a) shows that $T_1$ is traversing the vertex list looking for $7$. Meanwhile, $T_2$ and $T_3$ searching for the presence of vertex $7$ in vertex list. Suppose $T_2$ has reached Line \ref{lin:helploce16} and before it could $read(v_2.val)$ i.e. vertex 9, $T_1$ adds $7$, which is shown in the Figure (b), so $T_2$ and $T_3$ returns $false$ and $T_1$ successfully add the vertex $7$. This situation precisely shows why the $\lp$ must be re-ordered. Figure (c) depicts the correct $\lp$ order.}  
  \label{fig:lpcase3}
\end{figure}
}
\noindent We linearize a successful $\reme(u,v)$ method call within its execution interval at the earlier of the following points; (1) if there is no successful concurrent delete vertex, the $LP$ is later of $read(e_2.val)$ in Line \ref{lin:reme3} and $write(e_2.marked, true)$ in Line \ref{lin:reme4}, based on the execution. If the last line to execute is \ref{lin:reme4}, the edge $(u,v)$ is already present in the edge list of the vertex $u$, the $\lp$ is the logically marked as deleted. If the last line to execute is \ref{lin:reme3}, the edge $(u,v)$ is not present in the edge list of the vertex $u$, the $\lp$ is the $read(e_2.val)$. (2) if there is a successful concurrent delete vertex on $u$ or $v$ or both, it is linearized just before the $LP$ of the first successful concurrent delete vertex on $u$ or $v$. \\
Figure \ref{fig:lpcase5} illustrates why a concurrent $\remv$ must be considered while linearizing a successful $\reme$ \mth. Suppose the point where the edge $(5, 9)$ is removed from the graph is considered as a LP while there is a concurrent $\remv(9)$. The example shown shows that this \lp will be wrong, since the $\reme$ returns true after successful deletion of the corresponding vertex. For an unsuccessful $\reme(u,v)$ method call, the $LP$s remain same as the $LP$s of the $\adde(u,v)$ returning unsuccessfully, as described in Figure \ref{fig:lpcase3}. \\
\ignore{
\begin{figure}[H]
\captionsetup{font=scriptsize}
 \centerline{\scalebox{0.5}{\input{figs/LPCase5.pdf_t}}}
\caption{An execution of two concurrent operations  $T_1.\remv(9, true)$ and $T_2.\reme(5, 9, true)$. Figure (a) shows that $T_2$ has validated vertices $5$ and $9$ for presence in the vertex list and proceeds to remove the edge $(5, 9)$. Meanwhile, when $T_1$ is traversing the vertex list and it finds vertex $9$ and has marked it (logically removal). Then $T_1$ removes the $\enode$ $9$ from $5$'s list. Figure (b) shows that $T_2$ has now removed the edge $(5, 9)$. The actual sequence: $T_1.\remv(9, true)$ $<_H$ $T_2.\reme(5, 9, true)$  (ordered by their execution) is not linearizable. Figure (c) depicts the correct $LP$ order.}
\label{fig:lpcase5}
\end{figure}
}
%If the $\reme$ $(u,v)$ method returns unsuccessfully, it is linearized within its execution interval at the earlier of the following points: (1) if no successful concurrent add vertex on $u$ and $v$, then $LP$ is last of ($read(v_1.val)$ \vee $read(v_1.marked)))$ in Line \ref{lin:helploce8} and ($read(v_2.val)$ \vee $read(v_2.marked)))$ in Line \ref{lin:helploce16}, based on the execution. If the last line to execute was \ref{lin:helploce8}, then key $u$ was not present in the vertex list or it was marked and  similarly Line \ref{lin:helploce16} implies that the key $v$ was not present earlier or it was marked (2) if there is a successful concurrent add vertex on $u$ or $v$, then linearized at the point immediately before the $LP$ of the first successful concurrent add vertex $u$ or $v$.  
We linearize a successful $\cone(u, v)$ method call within its execution interval at the earlier of the following points: (1) if there is no successful concurrent delete vertex on $u$ and $v$, the $LP$ is $read(e.marked)$ in Line \ref{lin:cone151} where the edge node with key $v$ is found to be unmarked in the edge list of vertex $u$. (2) if there is a successful concurrent delete vertex on $u$ or $v$, it is linearized immediately before the $LP$ of the first successful concurrent delete on corresponding vertex. Figure \ref{fig:lpcase4} illustrates why a concurrent $\remv$ must be considered while linearizing a successful $\cone$ \mth. If the $\cone(u, v)$ method returns unsuccessfully, it is linearized within its execution interval at the earlier of the following points; (1) if there is no successful concurrent add edge (u, v), the $LP$ is, (a) last of $read(u.val)$ in Line \ref{lin:helploce8}/\ref{lin:helploce8.1} where $u$ is not found in the vertex list, (b) $read(u.marked)$ in Line \ref{lin:helploce8}/\ref{lin:helploce8.1} where $u$ is found to be marked, (c) $read(v.val)$ in Line \ref{lin:helploce16}/\ref{lin:helploce16.1} where $v$ is not found in the vertex list, (d) $read(v_2.marked)$ in Line \ref{lin:helploce16}/\ref{lin:helploce16.1} where $v$ is found to be marked, depending upon the execution. (2) if there is a successful concurrent add edge on $(u,v)$, it is linearized immediately before the $LP$ of that successful concurrent add edge. Figure \ref{fig:lpcase6} illustrates why a concurrent $\adde$ must be considered while linearizing an unsuccessful $\cone$ \mth. Suppose the point where the edge $(5,9)$ is added to the graph is considered as a LP while there is a concurrent $\cone(5,9)$. The example shown shows that this \lp will be wrong, since the $\cone$ returns false after the successful addition of the corresponding edge.

%The example shown shows that this \lp will be wrong, since the $\cone$ returns true after the successful deletion of the corresponding vertex.
\ignore{
\begin{figure}[H]
\captionsetup{font=scriptsize}
 \centerline{\scalebox{0.5}{\input{figs/LPCase4_1.pdf_t}}}
 \caption{An execution of three concurrent operations $T_1:\remv(9, true)$, $T_2:\cone(5, 9, true)$. Figure (a) shows that $T_2$ has validated vertices $5$ and $9$ for presence in the vertex list and proceeds to find the presence of the edge $(5, 9)$. Meanwhile, $T_1$ is traversing the vertex list and upon finding vertex $9$, marks it for logical removal. Figure (b) depicts that $T_2$ is on the process of searching the edge $(5, 9)$. The sequential history: $T_1.\remv(9, true)$ $<_H$ $T_2.\cone(5, 9, true)$ (ordered by their execution) is not linearizable. Figure (c) depicts the correct $LP$ order.}
\label{fig:lpcase4}
\end{figure}
}
\ignore{
\begin{figure}[h]
\captionsetup{font=scriptsize}
\centerline{\scalebox{0.45}{\input{figs/LPCase6.pdf_t}}}
 \caption{an execution of three concurrent operations $T_1:
 	\cone(5, 9, false)$, $T_2:\adde(5,9, true)$ and $T_3:\reme(5,9, true)$. Figure (a) shows that $T_1$, $T_2$ and $T_3$ have validated vertices $5$ and $9$ for presence in the vertex list. $T_1$ proceeds to find the presence of the edge $(5, 9)$. Meanwhile, $T_3$ proceeds to find the presence of the edge $(5, 9)$ and removes it by logically marking. After $T_3$ has released locks on edge nodes, $T_2$ proceeds to find the presence of the edge $(5, 9)$, and finds that edge node $9$ is not present, so it adds a new $\enode$ in the edge list. Figure (b) depicts that $T_1$ is still pointing to the removed edge node $9$ and after reading that it is marked, it returns $false$. The sequential history: $T_3.\reme(5, 9, true)$ $<_H$ $T_2.\adde(5, 9, true)$ $<_H$ $T_1.\cone(5, 9, false)$ (ordered by their execution) is not linearizable. Figure (c) depicts the correct $LP$ order.}
\label{fig:lpcase6}
\vspace{-5mm}
\end{figure}
}
As is evident, the $LP$ of the methods have been defined in a dependent manner. To make the LPs precise, we define a total order on overlapping \mth{s}. Given a history, we first linearize all the vertex \mth{s} as follows: $\addv \rightarrow \remv \rightarrow \conv$. Since the $LP$ of $\conv$ is dependent on $\remv$, this ordering does not cause any ambiguity. After ordering the LPs of vertex \mth, we order the LPs of the edge \mth{s}, following a similar order: $\adde \rightarrow \reme \rightarrow \cone$. Thus with this order, by the time $\cone$'s $LP$ needs to be fixed, all the other \mth{s} on whose $LP$s it could possibly depend on have already been fixed. An example of this is illustrated in Figure \ref{fig:lpcase2}. 
\ignore{
\figref{lpcase6} shows an execution of three concurrent operations $T_1:\cone(5, 9, false)$, $T_2:\adde(5,9, true)$ and $T_3:\reme(5,9, true)$. Figure (a) shows that $T_1$, $T_2$ and $T_3$ have validated vertices $5$ and $9$ for presence in the vertex list. $T_1$ proceeds to find the presence of the edge $(5, 9)$. Meanwhile, $T_3$ proceeds to find the presence of the edge $(5, 9)$ and removes it by logically marking. After $T_3$ has released locks on edge nodes, $T_2$ proceeds to find the presence of the edge $(5, 9)$, and finds that edge node $9$ is not present, so it adds a new $\enode$ in the edge list. Figure (b) depicts that $T_1$ is still pointing to the removed edge node $9$ and after reading that it is marked, it returns $false$. The sequential history: $T_3.\reme(5, 9, true)$ $<_H$ $T_2.\adde(5, 9, true)$ $<_H$ $T_1.\cone(5, 9, false)$ (ordered by their execution) is not linearizable. Figure (c) depicts the correct $LP$ order.
}
%\ignore {
%\vspace{-5mm}

%\vspace{-7mm}
%}

%\noindent As is evident, the $LP$ of the methods have been defined in a dependent manner. To make the LPs precise, we define a total order on overlapping \mth{s} by linearizing all vertex operations before linearizing all edge operations. All calls on vertex/edge are linearized in the following order; all $Add$ methods followed by all $Remove$ methods which will be followed by linearizing all $Contains$ operations. An example of this is illustrated in Figure \ref{fig:lpcase2}.
%\Comment{Talk about how all histories are linearizable and proof in technical report.}
%\vspace{-.4cm}
\ignore{
\begin{figure}[H]
\captionsetup{font=scriptsize}
\centerline{\scalebox{0.5}{\input{figs/LPCase2.pdf_t}}}
\caption{Figure (a) shows an example of an execution with four concurrent operations and $T_1:\remv(7, true)$ linearize first. Figure (b) $T_2:\adde(5, 7, true)$ linearize before $T_1:\remv(7, true)$. Figure (c) $T_3:\reme(5, 7, true)$ linearize before $T_1:\remv(7, true)$ and after $T_2:\adde(5, 7, true)$.  Figure (d) $T_4:\cone(5, 7, true)$ linearize before $T_1:\reme(5, 7, true)$ and after $T_2:\adde(5, 7, true)$. The finally $LP$ order, we obtain $T_2$ $<_H$ $T_4$ $<_H$ $T_3$ $<_H$ $T_1$ }
\label{fig:lpcase2}
\end{figure}
}
%\Comment{Add an example figure to show this effect. }
%\noindent \textbf{Lemma 1}: The methods $\addv$, $\remv$, $\adde$ and $\reme$ are deadlock-free.\\[0.1cm]
%\noindent \textbf{Lemma 2}: The methods $\conv$ and $\cone$ are wait-free.




 
 %\begin{figure}[tbph]
%\centerline{\scalebox{0.5}{\input{figs/LPCase1.pdf_t}}}
%\caption{Concurrently $T_1$ is doing $\adde(u,v)$ and retuning $true$, $T_2$ is doing $\remv(u)$ and returning $true$ and $T_3$ is doing $\cone(u,v)$ and retuning $true$ .}

%\end{figure}

%\begin{figure}[tbph]
%\centerline{\scalebox{0.5}{\input{figs/LPCase1a.pdf_t}}}
%\label{fig:LPCase1}
%\end{figure}
%\begin{figure}[tbph]
%\centerline{\scalebox{0.5}{\input{figs/LPCase1b.pdf_t}}}
%\end{figure}
%\begin{figure}[tbph]
%\centerline{\scalebox{0.5}{\input{figs/LPCase1c.pdf_t}}}
%\end{figure}
%\begin{figure}[tbph]
%\centerline{\scalebox{0.5}{\input{figs/LPCase1d.pdf_t}}}
%\caption{(a). $T_1$ is doing $\adde(5,7)$ and $T_2$ is doing $\remv(7)$ (b). $T_1$ and $T_2$ while running.}, (c). After finishing both the threads $T_1$ and $T_2$ The $LP$ of $\adde(5,7)$ just before $\remv(7)$ .}

%\end{figure}

%\subsection{Proof Outline}


